Stack Attention: Improving the Ability of Transformers to Model Hierarchical Patterns

Attention, specifically scaled dot-product attention, has proven effective for natural language, but it does not have a mechanism for handling hierarchical patterns of arbitrary nesting depth, which limits its ability to recognize certain syntactic structures. To address this shortcoming, we propose stack attention: an attention operator that incorporates stacks, inspired by their theoretical connections to context-free languages (CFLs). We show that stack attention is analogous to standard attention, but with a latent model of syntax that requires no syntactic supervision. We propose two variants: one related to deterministic pushdown automata (PDAs) and one based on nondeterministic PDAs, which allows transformers to recognize arbitrary CFLs. We show that transformers with stack attention are very effective at learning CFLs that standard transformers struggle on, achieving strong results on a CFL with theoretically maximal parsing difficulty. We also show that stack attention is more effective at natural language modeling under a constrained parameter budget, and we include results on machine translation.

==> figures/01-cfls/test/dyck.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={Dyck},
x grid style={white!69.0196078431373!black},
xmin=37, xmax=103,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.14622074019474,
ytick style={color=black},
ytick={0.0, 0.1}
]
\addplot [dashedline]
table {%
80 0
80 0.14622074019474
};
\addplot [cedline, color0]
table {%
40 0.0935325731881225
42 0.0775122494694571
44 0.0707845466828101
46 0.0662733913689785
48 0.061631194753904
50 0.0619074512276716
52 0.0573287197701992
54 0.0580696380992898
56 0.0554930854531065
58 0.05388274752278
60 0.0566759658028534
62 0.0524571667286687
64 0.054971859080852
66 0.0542708366604868
68 0.0586735043860551
70 0.0572370064603536
72 0.0630635394363194
74 0.064230935304154
76 0.0618965628987725
78 0.070193312273059
80 0.0713941330238577
82 0.0747885126217596
84 0.0823747876918149
86 0.0822633980395836
88 0.0928469879590642
90 0.0932211595501405
92 0.102587996458445
94 0.11757937144243
96 0.116163835011295
98 0.112260369350269
100 0.137598127596016
};
\addplot [cedline, color1]
table {%
40 0.108354470771149
42 0.0953710662357463
44 0.085481500070302
46 0.0774508840865902
48 0.0705421418058795
50 0.0635459300004891
52 0.0590551616978398
54 0.0549484900192347
56 0.0517389622335853
58 0.0480161284797824
60 0.0459097244365884
62 0.044176152133618
64 0.0432427501328883
66 0.0417245674022745
68 0.041343744674385
70 0.0424138199911558
72 0.0419486161522681
74 0.0434261300386573
76 0.0451220380956948
78 0.0457805343774397
80 0.0476129444315554
82 0.0506042945098143
84 0.0514825066726665
86 0.053420730184592
88 0.0554126248126684
90 0.0582485005770509
92 0.0610705410195956
94 0.0631660478933677
96 0.06594307439268
98 0.0692214543110344
100 0.0718381745698045
};
\addplot [cedline, color2]
table {%
40 0.0926947812340059
42 0.0793308854466805
44 0.0708538686606166
46 0.0669775136177889
48 0.0599754348638339
50 0.0576229190925329
52 0.0540548651666535
54 0.052504614447574
56 0.0497014108917438
58 0.0486191812254243
60 0.0481953191146208
62 0.0472333538423424
64 0.0472119470245084
66 0.046870977495619
68 0.0468350766335436
70 0.0482506458145417
72 0.0492460341044
74 0.0513031295174525
76 0.0528409707234589
78 0.0542288515579223
80 0.0553381953173281
82 0.0597268450158539
84 0.0622917142855378
86 0.0644223181194551
88 0.0687432281208461
90 0.071748048303051
92 0.0747356409873305
94 0.0769936363945587
96 0.0798810925811142
98 0.0834910668125632
100 0.0853908064119309
};
\addplot [cedline, color3]
table {%
40 0.0974552274090121
42 0.0730834181070904
44 0.0676441593081069
46 0.0645671152968467
48 0.0612205275314973
50 0.058513692407982
52 0.0573390720274186
54 0.05448874172646
56 0.0545199550499371
58 0.0543223995133681
60 0.0544263274508191
62 0.0532340344333245
64 0.0560119440892179
66 0.0541213511198523
68 0.0550250622757288
70 0.0563420074968778
72 0.0574900705863106
74 0.0595208817666854
76 0.0609697627464357
78 0.0648513802985604
80 0.063509085437201
82 0.0665858617622168
84 0.0722765352222571
86 0.0780106473135378
88 0.078964453813155
90 0.0839991614380884
92 0.0922250099595419
94 0.10563745323135
96 0.103537610740454
98 0.109380470628695
100 0.12332819721449
};
\addplot [cedline, color4]
table {%
40 0.100040227191615
42 0.0838130283296528
44 0.0761978832929331
46 0.068539164107604
48 0.0632007284057682
50 0.0611206632371953
52 0.055686048558988
54 0.053141687458825
56 0.0509632359468858
58 0.0481311436366642
60 0.0475067324728884
62 0.046653655138454
64 0.0461220404613309
66 0.0450027491659006
68 0.0448492814630701
70 0.0440376187546681
72 0.0431327480653985
74 0.0447371588604515
76 0.0438302321950755
78 0.0452363424830403
80 0.0484326313271263
82 0.0503357533446095
84 0.055580993408469
86 0.0579401060011626
88 0.0641406083052117
90 0.0655980080321825
92 0.0731362471996175
94 0.0753332367937006
96 0.0827181224772887
98 0.0831123573345129
100 0.084569996956942
};
\addplot [cedline, color5]
table {%
40 0.0943556949749026
42 0.0785748061286237
44 0.0719903509864273
46 0.0648363069114589
48 0.0600029728201679
50 0.0556205668149641
52 0.0528353064722459
54 0.0501147911832015
56 0.0481858970572134
58 0.0484586664653939
60 0.0460719905088099
62 0.0451378661304901
64 0.0452647922531628
66 0.0436941673781266
68 0.0456556524810323
70 0.0451005915580263
72 0.0468146399805743
74 0.0490379366743692
76 0.0510022127656594
78 0.0555101142846584
80 0.0628487508225567
82 0.0678245491147828
84 0.0765170686191387
86 0.0827070992513799
88 0.0919514919642785
90 0.0987750378335476
92 0.110989600427899
94 0.117677985237477
96 0.131114284133183
98 0.135955839328787
100 0.141226597550914
};
\end{axis}

\end{tikzpicture}


==> figures/01-cfls/test/hardest-cfl.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={Hardest CFL},
x grid style={white!69.0196078431373!black},
xlabel={Length},
xmin=37, xmax=103,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.315629153019341,
ytick style={color=black}
]
\addplot [dashedline]
table {%
80 5.55111512312578e-17
80 0.315629153019341
};
\addplot [cedline, color0]
table {%
40 0.143243741863653
41 0.133306365819466
42 0.128806829909666
43 0.12044877337407
44 0.115718906648582
45 0.116749102178379
46 0.114386782679135
47 0.112754051356728
48 0.10636848236486
49 0.106539377616663
50 0.108234097109197
51 0.100152705104327
52 0.0984383359835446
53 0.0972471955807421
54 0.0953227077410377
55 0.0949402686061493
56 0.102874163065036
57 0.0934429913141426
58 0.0936923660949154
59 0.091963130449729
60 0.100166410701619
61 0.102919856305365
62 0.090233496553445
63 0.09489066418704
64 0.0936584047618712
65 0.0913585869230276
66 0.0897252789405696
67 0.0858960863205627
68 0.0947889656494949
69 0.0910771372299333
70 0.0929820951677989
71 0.0956950493124702
72 0.0923895718392045
73 0.0964353674137861
74 0.0962374717889087
75 0.10328691730054
76 0.0993182648264432
77 0.0980567401760712
78 0.0996546103443416
79 0.105661586099665
80 0.103690945864352
81 0.109213911450547
82 0.102909452715717
83 0.112514919796525
84 0.112771274213213
85 0.115872952527497
86 0.118875686852489
87 0.118054070449405
88 0.121266104940629
89 0.124322931215944
90 0.123581678130814
91 0.131352942267666
92 0.134821721321047
93 0.133975058056458
94 0.134691236922907
95 0.148494507166109
96 0.146388718062097
97 0.150774900096595
98 0.147764274905356
99 0.147155805790414
100 0.152322256327241
};
\addplot [cedline, color1]
table {%
40 0.15055221293322
41 0.139790310558118
42 0.132612690184323
43 0.127972004027501
44 0.127515814949693
45 0.112770524168095
46 0.115378143000143
47 0.114471114457291
48 0.110325731730702
49 0.10529791874657
50 0.105791702596551
51 0.0998704853119226
52 0.100323326607016
53 0.094047757127629
54 0.0976487645898094
55 0.0956727398884079
56 0.105268039643624
57 0.0956656173637158
58 0.0919854378042253
59 0.0925799292343401
60 0.0977257378340008
61 0.101840674896558
62 0.0943730851549567
63 0.097745402413554
64 0.0931664158617123
65 0.0930073856628542
66 0.0871212155530392
67 0.0874401945354657
68 0.0979827978336645
69 0.0941183611459657
70 0.0871741675505573
71 0.0947260919222144
72 0.095091706401395
73 0.0945974693336313
74 0.10304264161028
75 0.102508360299616
76 0.10398653163679
77 0.0979586908571852
78 0.096971808990528
79 0.0996980683877535
80 0.104164499155128
81 0.106401137255422
82 0.104268212325674
83 0.10942870965648
84 0.110691253083691
85 0.112858090003667
86 0.118464172010727
87 0.112761435656425
88 0.117641224509035
89 0.115740690975205
90 0.122128541770149
91 0.128951786110183
92 0.127197535596366
93 0.136065332845152
94 0.129145402414353
95 0.138718592987971
96 0.13577787616813
97 0.138112092181055
98 0.13831868862213
99 0.139347631708536
100 0.144228888388378
};
\addplot [cedline, color2]
table {%
40 0.140503235845356
41 0.123956052463593
42 0.116637874716141
43 0.113294811497476
44 0.108702792147776
45 0.103481343400828
46 0.100423661149583
47 0.095150246586418
48 0.0909402450170806
49 0.0893229318966096
50 0.0938684765219167
51 0.0921307905936091
52 0.0880597699904151
53 0.0827912395048878
54 0.0826358640395999
55 0.0821986200645954
56 0.0799102633775537
57 0.0807362662170397
58 0.0847534272504873
59 0.0798124893345498
60 0.0799026030145649
61 0.0826405741572021
62 0.0755629608378845
63 0.0773266553365453
64 0.07838717593044
65 0.0722923683630563
66 0.0685803144903676
67 0.0752457733322853
68 0.0755275818203267
69 0.0742452466557071
70 0.0749632848282029
71 0.0754955994882298
72 0.0741789224155573
73 0.0777951279642051
74 0.0780614397097696
75 0.0740363010496916
76 0.0753629459174985
77 0.0763386359938056
78 0.0782996047044366
79 0.0818686838350506
80 0.0809370625176959
81 0.0797790967499485
82 0.0820557253337721
83 0.0846371081554542
84 0.084090460264449
85 0.0822597613382425
86 0.0926717673162165
87 0.0951236024048854
88 0.0927295951565461
89 0.0936553814953336
90 0.0947614589094921
91 0.0991500573528432
92 0.0955350834406932
93 0.105046811991532
94 0.103841399238943
95 0.109377449078084
96 0.112061102620757
97 0.106554196999506
98 0.110163966793896
99 0.10335034270596
100 0.113787817837231
};
\addplot [cedline, color3]
table {%
40 0.134679046764811
41 0.125683443482664
42 0.131136452771621
43 0.122751535127873
44 0.127494078236835
45 0.124865968201649
46 0.119770169329347
47 0.127393308100993
48 0.117974217131766
49 0.11598918073481
50 0.116545458156772
51 0.11019825443563
52 0.111161835522789
53 0.108155564151453
54 0.109030139431514
55 0.106716156804058
56 0.114443191152741
57 0.105299998991002
58 0.107822005507245
59 0.10176965915313
60 0.103535733393446
61 0.106088702558443
62 0.102581090962978
63 0.098875779486582
64 0.100770277081739
65 0.0999378862434452
66 0.103025533351873
67 0.0992586297088143
68 0.105397779486935
69 0.100574080661756
70 0.101341322691518
71 0.0976282338964929
72 0.0971781428974015
73 0.0956005231840662
74 0.0968333313138463
75 0.102183348277064
76 0.103027550910565
77 0.0992494125610761
78 0.0997672474541178
79 0.1010184191387
80 0.102115732240922
81 0.112793106058301
82 0.126585213865116
83 0.135544241040509
84 0.148470915183394
85 0.155479089022546
86 0.179964480127798
87 0.185441680697267
88 0.198844205270388
89 0.216112460541684
90 0.217640070379586
91 0.237665773381267
92 0.237838918239093
93 0.259283888236906
94 0.263307185160988
95 0.281175065745877
96 0.288452443097234
97 0.302317314016665
98 0.284998071630303
99 0.298961592984366
100 0.303521315884065
};
\addplot [cedline, color4]
table {%
40 0.145020400104136
41 0.135269545588161
42 0.139844465465165
43 0.131414074911244
44 0.140069314460357
45 0.133326491234996
46 0.12674205701429
47 0.132129081043936
48 0.12235236422913
49 0.122149860945411
50 0.12534768339223
51 0.1187431360742
52 0.122742852959255
53 0.116049834725222
54 0.117785023966165
55 0.112995742401014
56 0.117000500605155
57 0.11248687353635
58 0.110130414388738
59 0.104764568850873
60 0.108331151653436
61 0.112118811768461
62 0.109288807277168
63 0.105091369626642
64 0.110066321760188
65 0.104273073415918
66 0.10476012605079
67 0.102759951004956
68 0.108961908031435
69 0.105218993091727
70 0.109917378849877
71 0.103433222919685
72 0.101838032225781
73 0.101252327501545
74 0.10107334065156
75 0.106139479553928
76 0.105767715672751
77 0.10331297874443
78 0.0992606543650281
79 0.0983398787194654
80 0.107845710230177
81 0.128195046712056
82 0.147190514869258
83 0.162941509262204
84 0.165016908538999
85 0.170735615068456
86 0.180228967174825
87 0.187321298132689
88 0.196636535321572
89 0.201510225333443
90 0.200411153967661
91 0.208139934942701
92 0.207922579859167
93 0.221890597635004
94 0.226008818907659
95 0.241955794698111
96 0.237896623398062
97 0.240194668458823
98 0.226668599939351
99 0.227308361158659
100 0.244187295686869
};
\addplot [cedline, color5]
table {%
40 0.105318990756662
41 0.0974284399486134
42 0.0961044353209457
43 0.0909905494425256
44 0.0869658873267805
45 0.0872278347444904
46 0.0829915151787648
47 0.0819075705902581
48 0.0789631510851743
49 0.0806647067874204
50 0.0785874073541712
51 0.0768391144693952
52 0.0749794787863576
53 0.0737304934617751
54 0.0713574600430715
55 0.0698436595791874
56 0.0742939367319317
57 0.0713856633241234
58 0.0679196728057925
59 0.0677748512940628
60 0.0719613092997928
61 0.0738168928600511
62 0.068183998748143
63 0.068772934027127
64 0.0677220196534651
65 0.0701446535234582
66 0.0651065066799361
67 0.0636602995940758
68 0.0645097146011824
69 0.0672645043511695
70 0.0650876973626218
71 0.0655976136804701
72 0.0668755947472421
73 0.0667594351179941
74 0.0652883326929381
75 0.0684945752635253
76 0.0651835617916856
77 0.0643133494364272
78 0.0623808327929527
79 0.0613645731785388
80 0.0670584666311795
81 0.0766815788886337
82 0.0911659778520011
83 0.098905270585292
84 0.102741075709042
85 0.107828656942915
86 0.117686610022914
87 0.117436969851483
88 0.121537051717574
89 0.137273256218129
90 0.133495023591531
91 0.145738557935801
92 0.14422927413933
93 0.157960413828024
94 0.165313020001149
95 0.182848057687705
96 0.18612172991521
97 0.185055729573423
98 0.189913251495358
99 0.199898560008057
100 0.193292803782765
};
\end{axis}

\end{tikzpicture}


==> figures/01-cfls/test/marked-reversal.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={\MarkedReversal{}},
x grid style={white!69.0196078431373!black},
xmin=38.1, xmax=101.9,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=2.22446174145832,
ytick style={color=black}
]
\addplot [dashedline]
table {%
80 0
80 2.22446174145832
};
\addplot [cedline, color0]
table {%
41 0.0968068294264759
43 0.0683633498203935
45 0.0644592651753123
47 0.0628725093285751
49 0.0621814846823689
51 0.0558893578013063
53 0.0512445861244049
55 0.0509947678661618
57 0.0477232823934363
59 0.0473909610234066
61 0.0458928450858628
63 0.045217996598895
65 0.0446354189661712
67 0.0472686250100295
69 0.047716998101685
71 0.0507858058530481
73 0.0544964462928517
75 0.0631776372718366
77 0.068019350095557
79 0.0756104899677129
81 0.0923019055784834
83 0.101877895834019
85 0.116617802659977
87 0.14434047348548
89 0.173478765649954
91 0.189082293273634
93 0.225561811275751
95 0.261653684091209
97 0.31706314625301
99 0.354559865425274
};
\addplot [cedline, color1]
table {%
41 0.0767734026771072
43 0.0660754077195299
45 0.0635826728341634
47 0.0618401733729125
49 0.0589459631870638
51 0.0569164511188586
53 0.0544541160974709
55 0.0522303823260993
57 0.0501033822554925
59 0.048096217309227
61 0.0473977787494627
63 0.0456339276430691
65 0.0441434935768577
67 0.042878663180585
69 0.042307310960045
71 0.0421901475563545
73 0.0432906556901859
75 0.0452231409738216
77 0.0490446623593147
79 0.0536867629369949
81 0.0592209702543019
83 0.0652726376668398
85 0.0731512583047961
87 0.0809852721135871
89 0.0894738653221486
91 0.0975575970591064
93 0.108334580558114
95 0.116249325448826
97 0.12442604299119
99 0.134680970685954
};
\addplot [cedline, color2]
table {%
41 0.0705987956082328
43 0.067867390280525
45 0.0652407355148801
47 0.06231895044543
49 0.0593290375873337
51 0.0571184998321672
53 0.0552512155448896
55 0.0532109784713936
57 0.0517192425672861
59 0.0499931833584847
61 0.0477803628778309
63 0.0465783311869024
65 0.0449499060085128
67 0.0436763089894595
69 0.0419675277691387
71 0.0402085751495992
73 0.0391390109703561
75 0.0397237986832441
77 0.0434775014209636
79 0.0498733357837033
81 0.0588619633277027
83 0.0703043084120412
85 0.082617207148399
87 0.0960490026289488
89 0.109030282474642
91 0.121964262522405
93 0.134097869717884
95 0.146544558708112
97 0.158415938562415
99 0.168953404153438
};
\addplot [cedline, color3]
table {%
41 0.0715348961254045
43 0.0657762176949165
45 0.062880989927235
47 0.0605011620677433
49 0.0586503598652248
51 0.0573544675110954
53 0.0558082905673823
55 0.0546676284798129
57 0.0537713174822019
59 0.052700212947964
61 0.0522059597067157
63 0.0517080377672744
65 0.0508950300601251
67 0.0512833397084879
69 0.0496392624011603
71 0.0487778453265738
73 0.0458141472615068
75 0.043572838553149
77 0.042530618558347
79 0.0550496968512969
81 0.107131674453944
83 0.303244888104508
85 0.751944781246106
87 1.13780756775008
89 1.3277188400073
91 1.41383762349343
93 1.52692598802104
95 1.77568204732129
97 2.02417299401068
99 2.12032883733455
};
\addplot [cedline, color4]
table {%
41 0.0730212932372122
43 0.0690756612049226
45 0.0650256995965589
47 0.061962039343647
49 0.0583900631182101
51 0.0551545420703714
53 0.0532956459880712
55 0.0523535763762011
57 0.0514006713193574
59 0.0501012225359315
61 0.0486962792870855
63 0.0466280247803633
65 0.0442656622875979
67 0.0437360599145263
69 0.0438389415283377
71 0.0435990008314359
73 0.0432506471816501
75 0.0386300801750079
77 0.037670754859125
79 0.0411699999874211
81 0.107494380129217
83 0.169792130355986
85 0.230130138382929
87 0.287445425609146
89 0.340644869174594
91 0.391911058441491
93 0.442050185170202
95 0.489322692757546
97 0.534068303223525
99 0.57962574472598
};
\addplot [cedline, color5]
table {%
41 0.0752889997122192
43 0.0649492919060716
45 0.0613168801187656
47 0.0583968755728856
49 0.0570685908931897
51 0.0551533294570097
53 0.0531702445911101
55 0.0522102130181233
57 0.0515555135108823
59 0.0520682996559606
61 0.0522767494512933
63 0.0512653213394971
65 0.0501532727221565
67 0.0499076556923666
69 0.0488575365594157
71 0.0509970804942849
73 0.0486901299998662
75 0.0478816836938323
77 0.0532166412202062
79 0.078507114620483
81 0.180430409823741
83 0.552002181105667
85 1.08102818809113
87 1.38719503955394
89 1.54445082058932
91 1.62367703862209
93 1.64174699631671
95 1.71513272047049
97 1.68047124113025
99 1.71405997784359
};
\end{axis}

\end{tikzpicture}


==> figures/01-cfls/test/padded-reversal.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={\PaddedReversal{}},
x grid style={white!69.0196078431373!black},
xmin=37, xmax=103,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.736992455610046,
ytick style={color=black}
]
\addplot [dashedline]
table {%
80 0
80 0.736992455610046
};
\addplot [cedline, color0]
table {%
40 0.160194352774475
41 0.139309155476148
42 0.135651362384683
43 0.113756300028933
44 0.0979543137964931
45 0.0995347804617302
46 0.0961683262371232
47 0.10847851092255
48 0.114287825578872
49 0.0815903439783461
50 0.103622658915293
51 0.0894865556049925
52 0.086261358498507
53 0.0798756959473694
54 0.0995123531579435
55 0.0941587981885506
56 0.0818661599659246
57 0.095451976986425
58 0.0830412640611218
59 0.0846982156069556
60 0.0791542224022498
61 0.0893839569751997
62 0.0927194682795152
63 0.0879515451805413
64 0.0939195436848813
65 0.0928252182777816
66 0.105698790210922
67 0.0955491517066813
68 0.0928044039942728
69 0.1043478924499
70 0.11703842398503
71 0.0985675106562668
72 0.104098788212627
73 0.110234858013148
74 0.0978198960795097
75 0.105991518710908
76 0.136785635964588
77 0.123101633497224
78 0.137441540841282
79 0.1318320588216
80 0.13386632150262
81 0.127552016100664
82 0.128098069556027
83 0.150613193315292
84 0.146963226132751
85 0.151970345525043
86 0.165117929465488
87 0.16976710366699
88 0.183625739708171
89 0.191828816765302
90 0.20138355338227
91 0.207038647429263
92 0.207412619285244
93 0.203540846460054
94 0.23959354827347
95 0.232653533701848
96 0.190689125303496
97 0.240070203499318
98 0.252856846959706
99 0.269111133652333
100 0.268811768977087
};
\addplot [cedline, color1]
table {%
40 0.168147439369288
41 0.153018177044991
42 0.150699097247889
43 0.118991086104173
44 0.0989254927457848
45 0.112568968841985
46 0.109502079200418
47 0.11373929284142
48 0.111016923487174
49 0.0820494770603145
50 0.100623512696511
51 0.101519115931252
52 0.076233680897568
53 0.0780959560191894
54 0.0812099691411811
55 0.0746460942073895
56 0.0788185549849231
57 0.078393403660805
58 0.067048610362427
59 0.0642886133067589
60 0.0663960178318983
61 0.0740753508802302
62 0.0700702899584174
63 0.062201866610721
64 0.0642275410052358
65 0.07045892954658
66 0.0782565105236931
67 0.0670232947468094
68 0.0705963284128571
69 0.0767716063511153
70 0.0759319718193015
71 0.0828323532734154
72 0.0731094018443847
73 0.0866278224104637
74 0.0812181851532185
75 0.0958816769549796
76 0.115429664414283
77 0.0959570662147951
78 0.115174748982772
79 0.107052941400402
80 0.114495300006334
81 0.105418423428645
82 0.118765361111176
83 0.131250720045933
84 0.137330959554368
85 0.139702714070422
86 0.153032329005683
87 0.152841196397554
88 0.169891802512304
89 0.191337600189794
90 0.186708028864728
91 0.193267539253915
92 0.206318924766727
93 0.185343669760404
94 0.209400135962689
95 0.226100024565021
96 0.189930936818347
97 0.218549165193522
98 0.237139771615751
99 0.276444004145629
100 0.248377644757062
};
\addplot [cedline, color2]
table {%
40 0.117613073116164
41 0.103338015608686
42 0.0931483136444276
43 0.0863537566852363
44 0.0823291975229126
45 0.0799375499292453
46 0.0769599072882975
47 0.0768332404817085
48 0.0738127396829106
49 0.0728516718480769
50 0.0721355099537687
51 0.071297039165811
52 0.0698286834358193
53 0.0680552662247094
54 0.0685832845221718
55 0.0665973621171263
56 0.065485611222495
57 0.0646503462523574
58 0.0654397184017894
59 0.0621179929388195
60 0.063056361101147
61 0.0621119626343001
62 0.0614051866791772
63 0.0599530750164791
64 0.0585873909598487
65 0.0586505017406325
66 0.0571387448458382
67 0.0591559895004458
68 0.0574220599079452
69 0.055013376396091
70 0.0557522320769151
71 0.0557803476803217
72 0.0536732720177205
73 0.0544498423414955
74 0.0527712846323839
75 0.0522921010950134
76 0.0526093526059853
77 0.0532260604999316
78 0.0556159329505229
79 0.0575506333256219
80 0.0565300649249567
81 0.0590362550500322
82 0.0567122838643479
83 0.0621714752905876
84 0.0667089181427211
85 0.0695988079194348
86 0.0721368404760203
87 0.0782505795637301
88 0.0895992996207808
89 0.0927054955511227
90 0.0933647096812725
91 0.0997861751471253
92 0.106002806767572
93 0.111838566092802
94 0.120086409599783
95 0.120170472416037
96 0.12223009339427
97 0.142177759916121
98 0.142009598023418
99 0.151993467359729
100 0.160003612700594
};
\addplot [cedline, color3]
table {%
40 0.152471576219917
41 0.134480483945464
42 0.130326601763294
43 0.109866047021699
44 0.0963997286604792
45 0.101457881658626
46 0.103322808656256
47 0.107726910448644
48 0.113060145217875
49 0.0827895592968182
50 0.0988825859207382
51 0.100157471680197
52 0.0914460294423533
53 0.0893805121043987
54 0.0961965330004614
55 0.093374796247864
56 0.0948226063915127
57 0.0973981828431503
58 0.0931725863016724
59 0.0886580827472278
60 0.0862127617174796
61 0.0962311975884119
62 0.0862864117153107
63 0.0833651637392915
64 0.0965480344005785
65 0.0891648010717373
66 0.102670976070294
67 0.0882061610084349
68 0.0902390719006825
69 0.0934936312767615
70 0.0998492342663239
71 0.0971337321644929
72 0.0853624777155812
73 0.0978376178419345
74 0.0814469561809746
75 0.0933659389850078
76 0.115155454072432
77 0.116031503356817
78 0.119400991322798
79 0.113560821900507
80 0.141222038113815
81 0.133660468224909
82 0.149440359023181
83 0.205902052278933
84 0.232153386152257
85 0.279471059705097
86 0.33285104168705
87 0.370088215904583
88 0.472308024724102
89 0.475282642631586
90 0.514577449805494
91 0.521023156673755
92 0.569407204617583
93 0.603558305396152
94 0.627266072521343
95 0.639783666187308
96 0.575473902189782
97 0.674209846559522
98 0.672425598180862
99 0.691680460319939
100 0.704109076785829
};
\addplot [cedline, color4]
table {%
40 0.160399994767641
41 0.143257386776033
42 0.136841930639496
43 0.113611122790645
44 0.105911853417247
45 0.10959321637155
46 0.1072278775569
47 0.111866557846084
48 0.111873002243372
49 0.0854274404589687
50 0.102338329049368
51 0.100271655956483
52 0.0959589997847228
53 0.0906938756890842
54 0.0938230739913152
55 0.0913208912188841
56 0.0908871065233996
57 0.096084504746491
58 0.0887448558696215
59 0.0858466804960352
60 0.0863102263497703
61 0.0960148699520411
62 0.081072340896384
63 0.079427569222928
64 0.089772682379404
65 0.0858527482929319
66 0.0993879810286277
67 0.0842220077532432
68 0.0851242781155009
69 0.0949773542898551
70 0.101075039641089
71 0.09328162953791
72 0.0845992997502092
73 0.0992639432456569
74 0.0818781884357487
75 0.0941778159769593
76 0.116410835825599
77 0.115830775294526
78 0.127516881142033
79 0.11718744740543
80 0.143407264243266
81 0.130043340998611
82 0.129899801002068
83 0.186288903177851
84 0.177744708146232
85 0.204877044310277
86 0.239399687261634
87 0.254873655551758
88 0.326768266221312
89 0.332818517870881
90 0.342664193383149
91 0.389880550224387
92 0.40959500167011
93 0.427282901574643
94 0.459940991027048
95 0.502897440105346
96 0.403340591674332
97 0.485917970668483
98 0.516963176527316
99 0.520440386562573
100 0.537287081016556
};
\addplot [cedline, color5]
table {%
40 0.142240653525506
41 0.122893841741482
42 0.106816066496559
43 0.0996733716193902
44 0.0923029337730756
45 0.0903080656164449
46 0.086291832516508
47 0.0859475980936379
48 0.0824273921015317
49 0.0792289531692978
50 0.0779967908204248
51 0.0751849342082118
52 0.0734657485700299
53 0.0717176755058378
54 0.0700150316746517
55 0.0700430629477001
56 0.0665729093688192
57 0.0667654743131535
58 0.0632096707540553
59 0.0628144349392111
60 0.0591860927051154
61 0.0579410752458667
62 0.0570123265894319
63 0.0562459661752654
64 0.0547922718402701
65 0.0555116316474611
66 0.0549883523202688
67 0.051156802225271
68 0.0526669137359567
69 0.0514422372856682
70 0.0512852004199616
71 0.0497337002981993
72 0.0482320626175754
73 0.0481604604431528
74 0.0465469758520765
75 0.0464415003014896
76 0.0494889371622603
77 0.0474783581535784
78 0.0507197353624658
79 0.0600281301437001
80 0.065179716884211
81 0.0758835538525696
82 0.0802983729580487
83 0.0916590820804685
84 0.0921161677509527
85 0.10576569536762
86 0.112876366776865
87 0.119710134955967
88 0.13003897864026
89 0.142297395493742
90 0.14005449661167
91 0.161621903023858
92 0.160915231739603
93 0.166350629694758
94 0.1793222577723
95 0.179417516492728
96 0.165213482646966
97 0.205590692853686
98 0.213498609565349
99 0.232988819001958
100 0.217743449887452
};
\end{axis}

\end{tikzpicture}


==> figures/01-cfls/test/unmarked-reversal.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={\UnmarkedReversal{}},
x grid style={white!69.0196078431373!black},
xmin=37, xmax=103,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.87515971225119,
ytick style={color=black}
]
\addplot [dashedline]
table {%
80 0
80 0.87515971225119
};
\addplot [cedline, color0]
table {%
40 0.137428997919087
42 0.0690640671874733
44 0.0677777095333238
46 0.0633119083171531
48 0.073201224146797
50 0.0708689291973124
52 0.0641999632215938
54 0.0580327664291342
56 0.0636244993948772
58 0.0681707382318157
60 0.074076100953931
62 0.0755776151038238
64 0.0728237583341183
66 0.0691460111182516
68 0.0763861821567787
70 0.0901550632806949
72 0.094738616008419
74 0.103888074341872
76 0.128368486469814
78 0.129958968375345
80 0.148626472851239
82 0.181361671985668
84 0.200336919975812
86 0.206778769850723
88 0.233247551621135
90 0.262352929461355
92 0.309229911823354
94 0.331865873669176
96 0.369194663877162
98 0.394118327656442
100 0.422309527487231
};
\addplot [cedline, color1]
table {%
40 0.177923978099849
42 0.0631667917849404
44 0.0602706128279407
46 0.0585013007665235
48 0.0652778849950765
50 0.0680934799286087
52 0.0590789898099831
54 0.0673945306584953
56 0.0622810827773813
58 0.0670279824925598
60 0.0744092722959819
62 0.0637523270570008
64 0.0646080733420396
66 0.0753405818879814
68 0.0785904366432554
70 0.0847662827843114
72 0.0950441073210845
74 0.106039277375089
76 0.11135845980403
78 0.133106074981324
80 0.130921628033895
82 0.167546512619711
84 0.165068692327496
86 0.184929396134108
88 0.199785625845081
90 0.23688942729607
92 0.261792439072939
94 0.293312611142798
96 0.295833913243031
98 0.343114574112703
100 0.351261998840847
};
\addplot [cedline, color2]
table {%
40 0.0905136104793942
42 0.0754135754456517
44 0.0651230968255047
46 0.0641274660413519
48 0.0616276813643044
50 0.0589412906319856
52 0.0591820777497251
54 0.0557079114626896
56 0.0543044822098465
58 0.0539965952806307
60 0.0528127587980405
62 0.0504194729399022
64 0.0485288298696904
66 0.0478143343035421
68 0.0460807674561646
70 0.0461617380825181
72 0.0452465930141588
74 0.0449696588871198
76 0.0442111389178114
78 0.0480950683472039
80 0.0544650342926238
82 0.0600034251377299
84 0.0640752193994319
86 0.0765348166021506
88 0.0918627949760211
90 0.0996700759477571
92 0.108603909245281
94 0.121603752099649
96 0.131064449103606
98 0.14114080267383
100 0.149939656834602
};
\addplot [cedline, color3]
table {%
40 0.193045472977671
42 0.149394891608718
44 0.144238901095158
46 0.146589352695337
48 0.14945935998656
50 0.155370224291545
52 0.154066488533969
54 0.164672206339604
56 0.1690347194868
58 0.162055614885017
60 0.174892470156464
62 0.167401658241601
64 0.173179324707844
66 0.176929946450805
68 0.167695500067521
70 0.1774938813061
72 0.172072469408324
74 0.188090952880341
76 0.188220820777226
78 0.213855061742466
80 0.241483777930921
82 0.364974210077053
84 0.485604219763308
86 0.59184567355776
88 0.660498292641679
90 0.712070702786629
92 0.759171575927801
94 0.761865958590986
96 0.808917847938546
98 0.809364977738607
100 0.835590732568648
};
\addplot [cedline, color4]
table {%
40 0.188236723336604
42 0.142210909189061
44 0.131173337084111
46 0.131902689369595
48 0.13793519059664
50 0.147956262612205
52 0.149498400494644
54 0.157421232676239
56 0.157801244711614
58 0.156094325429123
60 0.160714086059274
62 0.15781937805923
64 0.16536474136896
66 0.165679317162271
68 0.160024460485227
70 0.165134430341218
72 0.16829059486582
74 0.182809881938079
76 0.184833322460864
78 0.203946269055743
80 0.210821773260126
82 0.250696554233537
84 0.301916151529163
86 0.390891742927845
88 0.440992982706166
90 0.481580984081174
92 0.493527989446769
94 0.557234658290422
96 0.568266769328137
98 0.622736300212161
100 0.621697736703005
};
\addplot [cedline, color5]
table {%
40 0.116513097256484
42 0.0884300726164597
44 0.0778293210029316
46 0.0705162805238292
48 0.0689541939570803
50 0.0690977143508858
52 0.0666374243487778
54 0.0678181305623187
56 0.0661170987358533
58 0.0643117534542602
60 0.068487287623606
62 0.0623667793190648
64 0.0574485870926039
66 0.0575862304182108
68 0.0552062676075795
70 0.056401648462042
72 0.0584014989191388
74 0.0660901346646006
76 0.0729731384983333
78 0.080646458755933
80 0.100919703825428
82 0.112924616047863
84 0.140303130285807
86 0.155513746090665
88 0.186280697581674
90 0.210667959619757
92 0.224163426090703
94 0.257736069443385
96 0.301185418794922
98 0.318817302723705
100 0.326080516947324
};
\end{axis}

\end{tikzpicture}


==> figures/01-cfls/train/dyck.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={Dyck},
x grid style={white!69.0196078431373!black},
xmin=-2.85, xmax=81.85,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.389574592553349,
ytick style={color=black}
]
\addplot [cedline, color0]
table {%
1 0.371081396335626
2 0.293066000386862
3 0.224970883518854
4 0.177900972556986
5 0.145545372088967
6 0.122159689948997
7 0.101726979851988
8 0.0796250328553512
9 0.0669480100883367
10 0.118634041038479
11 0.0515318307632046
12 0.048255273238368
13 0.0465284490677821
14 0.0499356423511563
15 0.0339035227040608
16 0.034470902542032
17 0.0438460963292585
18 0.0404215030177391
19 0.0326921820619216
20 0.0221690696649754
21 0.0268726784448809
22 0.0258687384060734
23 0.0215426747496298
24 0.0247194091356973
25 0.0253783468346193
26 0.0261679865052047
27 0.0210543741880681
28 0.0306028285502722
29 0.0197505250228752
30 0.0165930101958109
31 0.0167410394013726
32 0.0150891192872581
33 0.0139458511745238
34 0.0202835477887646
35 0.0161914088698841
36 0.0150834621787477
37 0.0183248035375211
38 0.0154539352006715
39 0.0145524943902642
40 0.0151212934833082
41 0.0144500172197944
42 0.0121258380084533
43 0.0128488781643079
44 0.012110116506468
45 0.0108733722267661
46 0.0145580365846112
47 0.0133206579205282
48 0.0197314036365014
49 0.0153223293015917
50 0.0116291318833822
51 0.0128108426670258
52 0.0103550841521266
53 0.0130677313449924
54 0.0113718733319754
55 0.0118653966031347
56 0.011249548811021
57 0.011448052416264
58 0.0111495723024593
59 0.0141145639460325
60 0.0099688571146429
61 0.0113286947213985
62 0.0158142605669465
63 0.0119684936405932
64 0.0124307626140713
65 0.0122320994240465
66 0.0132175821233012
67 0.0130647789764399
68 0.0144279637973235
69 0.0136221497169584
70 0.0148380542929921
};
\addplot [cedline, color1]
table {%
1 0.00957712891876072
2 0.0123998475449107
3 0.00678871775835976
4 0.0067051838559824
5 0.00694359737934069
6 0.00461124990834105
7 0.00473888259915345
8 0.0099686816103931
9 0.00462983935641437
10 0.00256619640042843
11 0.00239770258404948
12 0.0027924318208794
13 0.0038755644846028
14 0.00364744065515532
15 0.0033173096292588
16 0.00322471112486589
17 0.00976774140744818
18 0.00708321656881938
19 0.00544471210057718
20 0.0042217392627234
21 0.0049218969718563
};
\addplot [cedline, color2]
table {%
1 0.299862617643337
2 0.177546556585979
3 0.0171992924977835
4 0.0146358777093782
5 0.0124504130671668
6 0.00903858801045643
7 0.00752848266588535
8 0.00823799945890069
9 0.00806226411067867
10 0.00714311224984676
11 0.00579717541419189
12 0.00598551655305801
13 0.0052901730558963
14 0.00858133930771376
15 0.00541955659805149
16 0.00492173554820685
17 0.00398377822973373
18 0.00354262706274011
19 0.00604927662936416
20 0.00840743774655339
21 0.00326125295713986
22 0.00504333730568596
23 0.00642227456904798
24 0.00411024367796853
25 0.00462199822549814
26 0.00433736633936921
27 0.00451221445609329
28 0.00555698604043287
29 0.00445808958930027
30 0.00560820598814749
31 0.00451458828669982
};
\addplot [cedline, color3]
table {%
1 0.230032967963254
2 0.153003139327338
3 0.125234834396289
4 0.0934501213213893
5 0.0943411529571112
6 0.0689250082946847
7 0.0771366576258811
8 0.0564370762804287
9 0.115022000389758
10 0.0795067778506576
11 0.0759676065639479
12 0.0649901608465061
13 0.0473496884541434
14 0.045361732615914
15 0.0377359600005277
16 0.0394828025685269
17 0.0455139017474275
18 0.0315157688945834
19 0.0602267568773867
20 0.0838737244671326
21 0.0576826800819136
22 0.0483674362540714
23 0.0537004419465389
24 0.0390857490772353
25 0.0258170864834986
26 0.037295509263968
27 0.0307842920436781
28 0.0862146488697819
29 0.0282532892127869
30 0.0282155110472104
31 0.0303099861307611
32 0.0381038074387223
33 0.0472255710969991
34 0.0226188873305092
35 0.024046186907462
36 0.0197369564609687
37 0.0255037736084964
38 0.0310372016432104
39 0.0239092805023836
40 0.0238453457524735
41 0.0309715319499921
42 0.0262843830828094
43 0.0257567480869911
44 0.0182701168531334
45 0.0179328360474458
46 0.0566757210711454
47 0.0186905665328195
48 0.0207772476592841
49 0.016422080080298
50 0.0302536077239527
51 0.0197489574800069
52 0.0208256665159241
53 0.0268089631660618
54 0.0246704976909188
55 0.0203277482567819
56 0.0155018693446615
57 0.0137386139679584
58 0.0206535128634175
59 0.0144698943627871
60 0.0132107662366038
61 0.018923231140142
62 0.0124989853177465
63 0.0182905367789911
64 0.0274603415853515
65 0.0429994622425758
66 0.0122551950576207
67 0.0128802212625285
68 0.0117729561918588
69 0.0158155238166483
70 0.0124258662170859
71 0.0185414927844305
72 0.0167824250078074
73 0.0203473110994452
74 0.0124948776448424
75 0.0166656748482827
76 0.0157591411198981
77 0.020316452869777
78 0.0134103540450545
};
\addplot [cedline, color4]
table {%
1 0.0143866357537711
2 0.0123539795600226
3 0.0106209366994229
4 0.00531590826339157
5 0.00389064517599991
6 0.00441586625513735
7 0.00484112517239899
8 0.00841946239871461
9 0.00274173285507695
10 0.0056438989330333
11 0.00523566906058059
12 0.0024359323076284
13 0.00425215672475665
14 0.00231712309389942
15 0.00321798787461669
16 0.00490316398811685
17 0.00390119259473554
18 0.0119377823237774
19 0.00251698983424686
20 0.00260646591624625
21 0.00603859930800121
22 0.00184352634098051
23 0.00275134323086579
24 0.00197379077737647
25 0.0020162981974805
26 0.00206842075198421
27 0.00203078355355746
28 0.00429930592200289
29 0.00222026118234886
30 0.00333894306501659
31 0.0149725973137332
32 0.00264621730984937
};
\addplot [cedline, color5]
table {%
1 0.0067175783618959
2 0.00594341788861152
3 0.00447793444063316
4 0.00374634657444761
5 0.00296548298001098
6 0.00264861431038566
7 0.00247914051303744
8 0.00255038247151251
9 0.00794216720475427
10 0.00165360065854681
11 0.00175322990570537
12 0.0056382809521921
13 0.00145478862526394
14 0.00304750766306716
15 0.0025164866801356
16 0.0119525804447307
17 0.00247176626419976
18 0.0012174719811745
19 0.00577509434095891
20 0.00192413581694273
21 0.00214438997875965
22 0.00156765204290943
23 0.00844158563452091
24 0.00720719138261861
25 0.00214855423090365
26 0.00401500991892212
27 0.00209037210811192
28 0.00290259283296812
};
\end{axis}

\end{tikzpicture}


==> figures/01-cfls/train/hardest-cfl.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={Hardest CFL},
x grid style={white!69.0196078431373!black},
xlabel={Epoch},
xmin=-8.95, xmax=209.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.162610173568961,
ytick style={color=black},
ytick={0.0, 0.1}
]
\addplot [cedline, color0]
table {%
1 0.1199388679196
2 0.0859978407461015
3 0.0712126704075731
4 0.0612672012869306
5 0.0526816044237846
6 0.0511508125377618
7 0.0466037231468741
8 0.0460445818898401
9 0.0472813767719822
10 0.042453007482919
11 0.041071894574058
12 0.0421051266949928
13 0.0412651338212229
14 0.0403951537346101
15 0.040661819834785
16 0.0399888455708377
17 0.0383524350971622
18 0.0439153996902955
19 0.0434073676826097
20 0.042346693124127
21 0.0427302439657231
22 0.0462888916543263
23 0.0470059420326463
24 0.0453640237102482
25 0.0457494621425354
26 0.0476661855003782
27 0.0501284041439847
};
\addplot [cedline, color1]
table {%
1 0.10813471253664
2 0.0741064525978272
3 0.0668316680160785
4 0.0584245375520236
5 0.0539623948333965
6 0.0499986237398429
7 0.0465303408487605
8 0.0530016830368205
9 0.0445445587825273
10 0.0415449916834856
11 0.0406674326215348
12 0.0458468245541415
13 0.0394146271741174
14 0.0415550339450335
15 0.0433857332588254
16 0.0421871659449393
17 0.0403045428942321
18 0.0461589249225887
19 0.044437139149478
20 0.0448167021668817
21 0.0525928282820636
22 0.0484337043839371
23 0.0488301756862017
};
\addplot [cedline, color2]
table {%
1 0.155354430906288
2 0.130037426628179
3 0.10236438316079
4 0.0934759849422877
5 0.0968771855650228
6 0.0865753650154792
7 0.0672010874700211
8 0.0584567638108535
9 0.0528511915232803
10 0.042552969033526
11 0.0389831765793891
12 0.0438913502554619
13 0.0341399126750683
14 0.031458178817356
15 0.0414049307713298
16 0.0296430594783721
17 0.0295462980142847
18 0.0271812905699458
19 0.0264088792027626
20 0.0270217085227964
21 0.0253361293334702
22 0.0249979448848472
23 0.0284882227156142
24 0.0250984534782512
25 0.0241775184828437
26 0.0257900577301784
27 0.026270968351618
28 0.0264888873951159
29 0.0300498598390577
30 0.0294205599475776
31 0.0267594591432556
32 0.0287433213821442
33 0.0288388430938078
34 0.0282523934889314
35 0.0281713177790048
};
\addplot [cedline, color3]
table {%
1 0.15320953573706
2 0.129748068361221
3 0.120360138720463
4 0.111076785967313
5 0.109748252049546
6 0.105899336771956
7 0.100018638841668
8 0.0993865519460124
9 0.0966021956196401
10 0.0929812256338716
11 0.0923630401406974
12 0.0899432559346434
13 0.0889487691997577
14 0.087142505607948
15 0.0890988851982948
16 0.0876719762171227
17 0.0864237565675945
18 0.0846141700677536
19 0.0872886409582716
20 0.0798794235335294
21 0.0798946773980598
22 0.0825894938579153
23 0.0798756622708987
24 0.0797110931805833
25 0.0784516351205382
26 0.0796489155864109
27 0.0765835262898116
28 0.0830109842922284
29 0.0787935029482265
30 0.0727591527298099
31 0.0737268678194107
32 0.0718940322006154
33 0.0734740123517725
34 0.0712658298347482
35 0.0720909555425755
36 0.0762625029375859
37 0.0703506854717066
38 0.067596303188429
39 0.0679445450227931
40 0.0663454188256711
41 0.070585455579484
42 0.0669992616842459
43 0.0657562130330103
44 0.065244375276839
45 0.0659987383617526
46 0.0660005393346488
47 0.0646536715363946
48 0.0651431214092921
49 0.0663982630047726
50 0.0642923961571804
51 0.0658829395898
52 0.0630213250923626
53 0.0663319690597259
54 0.0617793828440607
55 0.0602386613069175
56 0.0615728631517911
57 0.060552300201393
58 0.0616253217048908
59 0.0614305834054134
60 0.0618245965599948
61 0.0655218961417121
62 0.0591091087747608
63 0.0592028691398698
64 0.0595512734606856
65 0.0596263345918282
66 0.0593640225592869
67 0.0586397481502159
68 0.0598518039648479
69 0.0568449927707428
70 0.0584275619818873
71 0.0587871205963493
72 0.0600952324883908
73 0.0578417884248037
74 0.0574256872144407
75 0.0571976394550797
76 0.0580650976711776
77 0.0570618974962731
78 0.0563989555410016
79 0.0562531562894113
80 0.0560009793090512
81 0.0553780211626089
82 0.0559562505743738
83 0.0550573997068173
84 0.0545762746942222
85 0.0565662294494214
86 0.0571253885485987
87 0.0543200301796114
88 0.0546056352009565
89 0.0555954583752589
90 0.0553162393857829
91 0.0560516979895547
92 0.0572906174075092
93 0.0528445167162799
94 0.0526922935546845
95 0.0536490465909614
96 0.053111656358005
97 0.0531428841762631
98 0.0518405758313867
99 0.0533057681194533
100 0.0521884392519854
101 0.0525476708224768
102 0.0523386985892507
103 0.0523166820137757
104 0.0537420333166101
105 0.0526381832663085
106 0.0524756200673595
107 0.0521781275618156
108 0.0514946336230682
109 0.0508080907340267
110 0.0518082327810054
111 0.0500369019293587
112 0.0522505219726119
113 0.0502666959708686
114 0.0508241172326054
115 0.0511141632209622
116 0.0512704972044287
117 0.0505457144152812
118 0.0562510167437502
119 0.0495611088740999
120 0.0506077916185781
121 0.0511630874181972
122 0.0499641317774038
123 0.0500220469143053
124 0.0514099299370421
125 0.0495273996251995
126 0.0503098504607744
127 0.0492357079352135
128 0.0498274043008893
129 0.0521674935199596
130 0.0496813974742725
131 0.0490849815852956
132 0.0486109990465255
133 0.0482477621718223
134 0.0486142329764006
135 0.0479934501911279
136 0.048472900482418
137 0.0488242004386825
138 0.0484677254582491
139 0.0497055180660335
140 0.0498071627393857
141 0.0500269986105089
142 0.0483455655479714
143 0.0479827715557604
144 0.0479136273288039
145 0.0485631356615532
146 0.0469398149038573
147 0.0476367867960283
148 0.0485313332718975
149 0.0480633438977136
150 0.0476351682511293
151 0.0471446284548735
152 0.0477368077875724
153 0.0477546098279131
154 0.0468848525214909
155 0.0465190435685063
156 0.049432835347808
157 0.0470705678797669
158 0.047455709326319
159 0.0466368903512988
160 0.047297374563019
161 0.0495037055433662
162 0.0477012027561245
163 0.046590228574749
164 0.0460061241082514
165 0.046737443398543
166 0.0472760023065601
167 0.0464702157177821
168 0.0467540752589024
169 0.0471706455182903
170 0.0462843888210513
171 0.0464330531008641
172 0.0454415762288527
173 0.0458690705413853
174 0.0465409721150405
175 0.0465190435685063
176 0.0457948073321073
177 0.0472945681311521
178 0.0467640110434946
179 0.0458274535561149
180 0.0452086154586522
181 0.0468809650873303
182 0.0456884294596422
183 0.0454985644038217
184 0.0458229134165791
185 0.0458956612666717
186 0.0453800426553748
187 0.0456779424102562
188 0.0456392366780405
189 0.0451145072796084
190 0.0448192530004012
191 0.0449317823176532
192 0.0453097448359301
193 0.0461715793729458
194 0.0455025653491261
195 0.0460409249415727
196 0.045280650907912
197 0.0454500111160652
198 0.045044515339471
199 0.0452810835375768
200 0.0452863832357806
};
\addplot [cedline, color4]
table {%
1 0.135038448343972
2 0.113393203259552
3 0.108695947871741
4 0.0962295662773429
5 0.0959509676104382
6 0.0997211309309696
7 0.0934195408897287
8 0.0861055823104879
9 0.0846841519571733
10 0.0840310455331632
11 0.0812165281000141
12 0.0788152711737442
13 0.0885979861230217
14 0.079834558029982
15 0.0774226714563984
16 0.0798473628130996
17 0.0746925435609975
18 0.0775530035890832
19 0.0745004037127368
20 0.0752747027981429
21 0.0730470667105494
22 0.0756234175577637
23 0.0735704736752814
24 0.073213601664069
25 0.0746389657902344
26 0.0714344675936105
27 0.0704859185078655
28 0.0688888626566944
29 0.0744842857290964
30 0.0701482317660183
31 0.0667442990873377
32 0.0675234653809083
33 0.0686954990691289
34 0.0691102848786238
35 0.0682617950027542
36 0.0687104473973903
37 0.068680024155884
38 0.0676115710149834
39 0.0649048946905546
40 0.070590259881411
41 0.0644574913899263
42 0.0669452112715128
43 0.0674019385334703
44 0.0647501811095745
45 0.0617649377579745
46 0.0653742785486175
47 0.0636539248567416
48 0.061541988969384
49 0.0632640714531902
50 0.0614152793234135
51 0.0600387828747233
52 0.059842319553687
53 0.0614037209081104
54 0.0604934739476866
55 0.0660572013664513
56 0.0615197231650888
57 0.0598568697824844
58 0.0619399331066293
59 0.0606256066390294
60 0.0595445775100722
61 0.0591738428471242
62 0.0563560644697798
63 0.0566320627059957
64 0.0578473599242559
65 0.0584032442076148
66 0.0558677126527543
67 0.0565393613698153
68 0.0563770600626778
69 0.0594235645946379
70 0.0566736156879715
71 0.0559380858396608
72 0.0575195359466161
73 0.0554001383458904
74 0.0551263608604045
75 0.0562570488543821
76 0.0558524644761507
77 0.0571179115558456
78 0.0631723004684122
79 0.0598381774790397
80 0.0550320257680004
81 0.0543975939040278
82 0.0543792264287253
83 0.0540906419198441
84 0.0567732292672705
85 0.0553717611532569
86 0.0574223388996478
87 0.0550208202166207
88 0.052690327144032
89 0.0536237319386563
90 0.0549472873402146
91 0.0535173912948468
92 0.0530493580724083
93 0.054633030786009
94 0.0551113147962385
95 0.0576933599010698
96 0.0526554545978364
97 0.0527739735094965
98 0.0546816061013777
99 0.0529417799645564
100 0.055478331480733
101 0.0537059110816467
102 0.0543223064701857
103 0.0524726212571913
104 0.0531262383170301
105 0.0523024888284809
106 0.0534090083901237
107 0.0523010976893203
108 0.0556788534571735
109 0.054283646039164
110 0.0521827367632701
111 0.0520395291391567
112 0.0521111355147663
113 0.0528190027349154
114 0.0518855955358322
115 0.050539969572619
116 0.0552915325529129
117 0.0506346221673848
118 0.0522301470258457
119 0.0517951297563786
120 0.0524634198662406
121 0.0553855231254394
122 0.0500949930552115
123 0.0535588601472556
124 0.0520525877842475
125 0.0517737165397552
126 0.0518264992908353
127 0.0546452015261194
128 0.0526651890812437
129 0.0529824171904854
130 0.0503185782964071
131 0.053231230716404
132 0.0536054571151268
};
\addplot [cedline, color5]
table {%
1 0.123472423739393
2 0.109163938335656
3 0.0998593108913872
4 0.0949723534355302
5 0.0894961244641828
6 0.0842963205149676
7 0.083785755414634
8 0.0787505475096948
9 0.0784917251165327
10 0.0746479243509983
11 0.0655712521890714
12 0.0319390100448955
13 0.0261788086869952
14 0.0227985396391632
15 0.0230120216565564
16 0.0213368013928696
17 0.0214791136357317
18 0.0210570098468652
19 0.020158835010708
20 0.019388312346321
21 0.0185818518814742
22 0.0192005752545747
23 0.0207784750139168
24 0.0191001743696924
25 0.0190786665428764
26 0.0191163327953672
27 0.0183873837845567
28 0.0168825463486431
29 0.0178105590164785
30 0.0160897102556863
31 0.0177650324735477
32 0.0151776632330043
33 0.0147384523351699
34 0.0197051014353857
35 0.0160733910739521
36 0.0189827114832044
37 0.017279845212947
38 0.0152324811151483
39 0.0164965977114371
40 0.0132440269727461
41 0.0138782712298084
42 0.0143131571507884
43 0.0136903930887879
44 0.0139255432955663
45 0.0128396263666768
46 0.0140780980845367
47 0.0179322877045827
48 0.0148186996581336
49 0.0124257508767225
50 0.0124129617513382
51 0.0129590463891833
52 0.0130064740470177
53 0.0146695038851898
54 0.0161238008377191
55 0.0159383563928612
56 0.0115138353898951
57 0.0148492523855126
58 0.0113588674022655
59 0.0137036140528899
60 0.0143463006257594
61 0.0140080960230875
62 0.0124577229746194
63 0.0115664965793238
64 0.0123417210861492
65 0.0133954529240921
66 0.0142891946299615
67 0.0142588487445336
68 0.0108137058435132
69 0.0111902843714387
70 0.010973252246687
71 0.0117228918230941
72 0.0117561212583146
73 0.0102395776528408
74 0.0107288662276992
75 0.0138294285492722
76 0.0119965527160788
77 0.01044013286769
78 0.0104528348424371
79 0.0117871044666529
80 0.01095179361351
81 0.0108128069184252
82 0.0111566991470471
83 0.0103522262842284
};
\end{axis}

\end{tikzpicture}


==> figures/01-cfls/train/marked-reversal.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={\MarkedReversal{}},
x grid style={white!69.0196078431373!black},
xmin=-4.05, xmax=107.05,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.429929349396038,
ytick style={color=black}
]
\addplot [cedline, color0]
table {%
1 0.407271463429514
2 0.374268047633326
3 0.325369672695966
4 0.250981499565885
5 0.214070801145204
6 0.171873836104374
7 0.146228045402089
8 0.157730715157927
9 0.108240418082155
10 0.0938526313587473
11 0.115071428707996
12 0.0842684174849322
13 0.0736989048670592
14 0.077230172166891
15 0.0834772389827845
16 0.0447667923724854
17 0.0578153539565484
18 0.0591991574048976
19 0.0460665687404501
20 0.0428465623737418
21 0.0339379223400956
22 0.0314656819471877
23 0.0231760977472478
24 0.0317716963750156
25 0.0226568848363306
26 0.0370627108988388
27 0.0270795503481849
28 0.0270946323474756
29 0.0376898269671221
30 0.0406269680019936
31 0.0290992232558714
32 0.0392936540114399
33 0.0338174554649289
34 0.0177060079045791
35 0.0138167744975903
36 0.0249865542887465
37 0.0420156863365355
38 0.0127135954505903
39 0.0231808541025511
40 0.0288525343633601
41 0.0142061472583612
42 0.0162380721562804
43 0.0232383249409717
44 0.0390534467376996
45 0.00940115792211355
46 0.0144264073308914
47 0.0131940390472535
48 0.0135484374760472
49 0.0154643515306332
50 0.0101005542482898
51 0.0134475023532724
52 0.0116513797571772
53 0.00836413909079048
54 0.0179425520656395
55 0.0113581560694357
56 0.0100786277077416
57 0.0102877535960239
58 0.0130852206535546
59 0.00678483452439382
60 0.00734545350946758
61 0.0121041997034873
62 0.0088338900349087
63 0.0101051322565261
64 0.0102907247317217
65 0.0115450399647106
66 0.0063062995721157
67 0.0126231510967778
68 0.00946754324683413
69 0.0128888531631792
70 0.011855687229728
71 0.0116255577098948
72 0.00998368746821365
73 0.00789730661943794
74 0.00804049389354539
75 0.0103629928812766
76 0.00611980480046365
77 0.0100403956665556
78 0.00553388984332248
79 0.00885101890427947
80 0.00581333924592214
81 0.0123976054064545
82 0.00800636905167124
83 0.0101113165501631
84 0.0122626542835589
85 0.0109117392031904
86 0.00851160351747721
87 0.0128605000217574
88 0.0108439248147569
};
\addplot [cedline, color1]
table {%
1 0.409449233272445
2 0.374345255167809
3 0.335225583865516
4 0.0365581672905618
5 0.0122811889753902
6 0.012456017089541
7 0.00605152184728452
8 0.00715470215667086
9 0.0126477805455845
10 0.00357326580064399
11 0.00562359322595096
12 0.01679912351319
13 0.00427156713238902
14 0.0055814431072897
15 0.00379968187101537
16 0.00438357287288099
17 0.0028882146397945
18 0.00359490835416898
19 0.00186097059244483
20 0.00448927283629103
21 0.00264922496447378
22 0.00292457938400126
23 0.00269877334073393
24 0.00235665359516379
25 0.00147033291354826
26 0.00233417565810706
27 0.00430255556660403
28 0.00132028360094416
29 0.00196103278558984
30 0.0026076767989891
31 0.00158912621649704
32 0.00124549333539659
33 0.0013709500181206
34 0.00138810803120043
35 0.00254082427905866
36 0.00422459845604889
37 0.00097501994095045
38 0.00175013820714076
39 0.00259724907012204
40 0.00185199119954477
41 0.00097121449556048
42 0.00152503784962227
43 0.0018168818083048
44 0.00147526942854914
45 0.0017066108892112
46 0.00313870050287413
47 0.00113515938728953
48 0.00228323457824703
49 0.00176275915689816
50 0.00227029674791779
51 0.00285265672232748
};
\addplot [cedline, color2]
table {%
1 0.33970017513394
2 0.273713009639104
3 0.0067687349364195
4 0.00641315233018092
5 0.00251411134139606
6 0.00192841181539988
7 0.00234781046741483
8 0.00217840301433753
9 0.00333411367862196
10 0.00405098368398649
11 0.00181648302241966
12 0.00235842279593518
13 0.00258409038739804
14 0.0020179620379191
15 0.00164333748887024
16 0.00122510304510048
17 0.00149213487038524
18 0.00255954968228406
19 0.00296467768677339
20 0.00209599790990644
21 0.00312205273604516
22 0.00134577490529092
23 0.00123524069039888
24 0.00423074756788472
25 0.00325957371701396
26 0.00108373301025938
27 0.00160028963428238
28 0.00301155278355297
29 0.000690500801575955
30 0.00308254939343394
31 0.00113499513737308
32 0.0069366408436986
33 0.000926766960071268
34 0.000925306695098105
35 0.00102184184581172
36 0.00136758835818335
37 0.00205094367383635
38 0.00110490328950791
39 0.000745353278045147
};
\addplot [cedline, color3]
table {%
1 0.349745124781062
2 0.311262193563994
3 0.242601404448114
4 0.217774474837381
5 0.21098088562758
6 0.135211960690662
7 0.106092586321036
8 0.104302808020191
9 0.0732230894784796
10 0.0724666122955007
11 0.0582641926450529
12 0.0455115894364237
13 0.0704144372245788
14 0.039965670198165
15 0.0353213342275283
16 0.0412037606544478
17 0.0436086056080933
18 0.0416452364773447
19 0.0600327358745147
20 0.0312543543863038
21 0.0302208640142393
22 0.0353377880483527
23 0.0389034403107425
24 0.0305999869959201
25 0.0333367428595568
26 0.0190828750289766
27 0.0244863679754752
28 0.0261661771574925
29 0.0301284039220441
30 0.0513790401555884
31 0.0247985482347872
32 0.0248562695241923
33 0.0355497830656186
34 0.0307301076072046
35 0.0278401695761637
36 0.0182099347771965
37 0.0190167758963404
38 0.0199564065324112
39 0.0298336401594364
40 0.0202456642844036
41 0.0149446987452413
42 0.0286347849823164
43 0.0233174004629698
44 0.0186398477194759
45 0.0312722126523273
46 0.0239828888289397
47 0.0156495026277926
48 0.0181258430741484
49 0.0163468629197949
50 0.0132729911441454
51 0.0162690031576447
52 0.0120395889473275
53 0.0173288925914562
54 0.0150329763226261
55 0.0161535199778092
56 0.0156833034634435
57 0.00927150534458732
58 0.0226578963537735
59 0.0131668544782294
60 0.0123836582870678
61 0.0183337080876127
62 0.0439673853753959
63 0.0184922876864964
64 0.0089010219737739
65 0.0116832870809624
66 0.0119077351566287
67 0.0102597010131378
68 0.0109484649051929
69 0.0121242741837422
70 0.0147523641768684
71 0.00854150742718435
72 0.0110106037981628
73 0.0078203185404917
74 0.0134982839506613
75 0.00864548060284248
76 0.0176941938861327
77 0.00835920637939819
78 0.0242579125525588
79 0.00938320255567876
80 0.00619779638910761
81 0.0138910033936995
82 0.00727155104623634
83 0.00871540694484418
84 0.00659307025447758
85 0.00849885276519635
86 0.0109595442154722
87 0.00787556528608185
88 0.0126436964718217
89 0.0046385670463282
90 0.00599731726349645
91 0.00503994936101593
92 0.0043294033462129
93 0.00530787870485461
94 0.00727735286481634
95 0.00447825990266953
96 0.0047038460600049
97 0.00695288281560813
98 0.00750504765905829
99 0.0100523203748762
100 0.00639186384598356
101 0.00583472620558995
102 0.00802115724811658
};
\addplot [cedline, color4]
table {%
1 0.330820285590337
2 0.00766635484584505
3 0.00275071650624492
4 0.00460240469384793
5 0.00376403331474789
6 0.00322693834208954
7 0.00121398618249852
8 0.000714836384123618
9 0.000706243542236473
10 0.00126502983893362
11 0.00107818116523434
12 0.000567856192419114
13 0.000563721302080655
14 0.00042628727779731
15 0.000909128390380709
16 0.000976315297695762
17 0.00172713991950829
18 0.000561207929010377
19 0.00413459321592308
20 0.000127191513100922
21 0.000300999099619115
22 0.000655414561681
23 0.000428557727801315
24 0.000220222476135401
25 0.000228008458933282
26 6.21376944269225e-05
27 0.000302702150964063
28 6.18943430205632e-05
29 0.00164753127007961
30 0.000521803899545981
31 -1.22494763919456e-05
32 0.000993982516504011
33 0.000301485686013625
34 0.000334167530169516
35 0.00118822029973442
36 0.000603366899630753
37 0.00047437106392556
38 0.00130286528061158
39 -0.00015308919939766
40 0.000496182339553175
41 -1.07081375420037e-05
42 -0.000111062366962733
43 -1.32229547843421e-05
44 -8.76157318884796e-05
45 0.000416799984506222
46 0.000169125459679065
47 0.000245688903072971
48 8.16056150662603e-05
49 -9.97040667873872e-05
};
\addplot [cedline, color5]
table {%
1 0.363662789477193
2 0.348090045619571
3 0.336126895834034
4 0.253099710363492
5 0.141866626497612
6 0.0766675221703501
7 0.0627425251184497
8 0.0406594282406738
9 0.0428067387700419
10 0.0265460893672573
11 0.0258948716100948
12 0.0428146567570847
13 0.0228089489862962
14 0.0172397966665642
15 0.0143628835786817
16 0.0122406339243168
17 0.0120738228183767
18 0.0219293322592684
19 0.0138313847943569
20 0.00944447606165766
21 0.0105363944825931
22 0.00729880172334357
23 0.00634295534434542
24 0.0151730493021964
25 0.0274346633095923
26 0.0402625197332994
27 0.0101979246125418
28 0.00973602231776066
29 0.00327789892291419
30 0.0180843982364024
31 0.00370323957526802
32 0.00601490189172088
33 0.00576713974404708
34 0.00682155604290435
35 0.0043539802797648
36 0.00603559965687434
37 0.0065917822427301
38 0.00530294406027343
39 0.00528674448603172
};
\end{axis}

\end{tikzpicture}


==> figures/01-cfls/train/padded-reversal.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={\PaddedReversal{}},
x grid style={white!69.0196078431373!black},
xmin=-7.25, xmax=174.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.267395555823754,
ytick style={color=black}
]
\addplot [cedline, color0]
table {%
1 0.254718881807881
2 0.223553094150216
3 0.208999603973524
4 0.207463135269279
5 0.212463644543286
6 0.20376713885399
7 0.207197482233921
8 0.194056822270274
9 0.189377256727462
10 0.181050881667326
11 0.178778667951053
12 0.169948422137377
13 0.159664502094444
14 0.149499999712523
15 0.141867404040707
16 0.135112474016707
17 0.122226859944863
18 0.122768665082682
19 0.112633793422162
20 0.109889111365883
21 0.10711871208691
22 0.104626447751239
23 0.102556408586754
24 0.0930760163740944
25 0.0891530440826315
26 0.0902137839901994
27 0.0840480527537803
28 0.0819780167532447
29 0.0866819806197305
30 0.0812979839184939
31 0.076409173821175
32 0.0799370099549953
33 0.0737418868528869
34 0.0738481928069223
35 0.0715119364714346
36 0.080585068406874
37 0.0636787884125604
38 0.0679907603402111
39 0.062759023570312
40 0.06694098480434
41 0.0632137987459269
42 0.0607823994844456
43 0.0658130918611393
44 0.0612628847004839
45 0.0678431300193991
46 0.0575179577820809
47 0.0586267646896402
48 0.0583409815633687
49 0.0554390832448742
50 0.0560812230391443
51 0.0584347785002718
52 0.0589641651580675
53 0.0546523617485305
54 0.0537957084373361
55 0.0528101799131857
56 0.0523444719061534
57 0.0530584633783009
58 0.0462701997256842
59 0.0521321681535337
60 0.0464823434512441
61 0.0501497552913351
62 0.0503077768257493
63 0.0494407028232421
64 0.0514199873606835
65 0.0518836545694882
66 0.0472450594292719
67 0.0452907399946414
68 0.0468789256943192
69 0.0474301861412555
70 0.0460164130687525
71 0.0511536543821367
72 0.0455923802132803
73 0.0425865104308957
74 0.0427641047910454
75 0.0419640160566201
76 0.0469747145251416
77 0.0464257706692889
78 0.0425098424448146
79 0.0415275232365711
80 0.0452947204469717
81 0.0459498693766826
82 0.0453693509946992
83 0.0435044065850832
84 0.0426803832896147
85 0.046399098350077
86 0.044040010713277
87 0.0459034601958775
88 0.0474823994151973
89 0.0455516748734678
};
\addplot [cedline, color1]
table {%
1 0.25186719498099
2 0.223906181571099
3 0.21722823194863
4 0.212698043980049
5 0.21439322726749
6 0.206893192723657
7 0.192886887072557
8 0.182093826046372
9 0.184644808370072
10 0.173228361473655
11 0.174019099259657
12 0.175034035681306
13 0.153734892482309
14 0.163614525207196
15 0.149984510503303
16 0.14060968081496
17 0.16206673342079
18 0.130804740996144
19 0.123405802359282
20 0.120918567351892
21 0.107236266812681
22 0.107377817317388
23 0.100163572478017
24 0.0981178631886611
25 0.103409459970778
26 0.0958936205473054
27 0.0808058641634739
28 0.0780606652869539
29 0.0854361830086217
30 0.0723244385323386
31 0.0711181839180376
32 0.068885206534139
33 0.069360025757217
34 0.0730428972771877
35 0.0622213473620345
36 0.0673448086655012
37 0.0551378578066269
38 0.0575070760224509
39 0.0563421247356046
40 0.0531084186654401
41 0.052042959423808
42 0.0447211851781878
43 0.0450747503260009
44 0.0415552701023522
45 0.0402710306500895
46 0.0433169310574006
47 0.039396751620162
48 0.0356390027774959
49 0.0373185090869973
50 0.0369746029335888
51 0.0315475939816551
52 0.0376730358765499
53 0.0367918989364244
54 0.0357599487822588
55 0.0322586146812787
56 0.034226020967223
57 0.0321498843695505
58 0.0346577986770641
59 0.0289812229512045
60 0.0301116202006712
61 0.0322646409578534
62 0.0333405860290154
63 0.0331535373789726
64 0.0307205599273292
65 0.0270449406073358
66 0.0298352864713243
67 0.0343777072622144
68 0.0294321418708886
69 0.0345349656188513
70 0.0299810968437674
71 0.0390713496013858
72 0.0337520200898062
73 0.0290477275940004
74 0.0311593837390707
75 0.032253843853235
};
\addplot [cedline, color2]
table {%
1 0.244712922816276
2 0.228601321664051
3 0.209236379981128
4 0.198886416094819
5 0.193117942987482
6 0.172393478533366
7 0.163570279756465
8 0.180931500709858
9 0.147563470670313
10 0.144244633312462
11 0.143766066755671
12 0.13684663218597
13 0.135745588827355
14 0.126301353369303
15 0.125282740095623
16 0.12367508337215
17 0.116267052018042
18 0.114580226921614
19 0.117607145726859
20 0.109038901045216
21 0.104535071272124
22 0.098716456338148
23 0.10118208770942
24 0.0928298278229579
25 0.0888601604485372
26 0.0888261446372219
27 0.0871846995555132
28 0.0889925567721181
29 0.0915760980746152
30 0.0798637139803963
31 0.0838620749544959
32 0.0783255514270946
33 0.0815566792699321
34 0.074531278431712
35 0.0804228240495302
36 0.0931619279461234
37 0.0768263647595444
38 0.0671304487211833
39 0.0675557111334577
40 0.0679988894336113
41 0.0728782135135048
42 0.0643522561628849
43 0.0565900686830108
44 0.0578853757411513
45 0.0478529492124804
46 0.0508517462288515
47 0.0586635902015664
48 0.0441012996721243
49 0.0438218352046861
50 0.0375733829768737
51 0.0396539463618045
52 0.034993164829128
53 0.0263456153686682
54 0.0188660747520453
55 0.00949723491868198
56 0.00659608949559981
57 0.00400120173593488
58 0.00439467384079911
59 0.00808777976556552
60 0.00694170435312824
61 0.00769213822886772
62 0.00404142966478982
63 0.00421945126400292
64 0.00757757892669736
65 0.00678599402147628
66 0.00327396513663231
67 0.00551922452478043
68 0.00508367709132934
69 0.00421824033977108
70 0.0054525352539968
71 0.00719717204885101
72 0.00365128027000416
73 0.00401141026680629
74 0.00322513488098064
75 0.0043727943180123
76 0.00434823333477607
77 0.0113788624820766
78 0.00576227445537669
79 0.00780461597099863
80 0.00792070041941956
81 0.00581754409133223
82 0.00637102190101757
83 0.00587022011995181
84 0.00581909850567902
};
\addplot [cedline, color3]
table {%
1 0.232916520949053
2 0.219484012787599
3 0.212260568058793
4 0.1977449120003
5 0.185488755305901
6 0.184049358991404
7 0.168244600638779
8 0.165802168877401
9 0.160711990585245
10 0.156897685313589
11 0.153237430628992
12 0.145457752345495
13 0.143745669317397
14 0.141588371408621
15 0.132389696878563
16 0.13374683154133
17 0.129390135407364
18 0.135929150071913
19 0.117504269849885
20 0.135711011917461
21 0.120600347358424
22 0.116109230079741
23 0.108204703955209
24 0.115284783230047
25 0.104085103690858
26 0.11828482066767
27 0.103829119714228
28 0.0998231090881928
29 0.0954787448724021
30 0.092551171360079
31 0.0945106139344821
32 0.0937628733419867
33 0.096997956315402
34 0.0912436848112324
35 0.0906308959012947
36 0.0850878208436303
37 0.0880675434136852
38 0.084123052637896
39 0.0856553255227976
40 0.0812885962690569
41 0.084619541454365
42 0.0804776602833055
43 0.0801151754962948
44 0.0794011244617207
45 0.0763899933611519
46 0.0825226706870019
47 0.0746808077200018
48 0.0741832827642354
49 0.0727603601380964
50 0.0710694566030329
51 0.0706053348302353
52 0.0816425480947574
53 0.0704235165163862
54 0.0670144585414187
55 0.0868860029802797
56 0.0681233392406969
57 0.0754053549507078
58 0.0686111635002465
59 0.0725980239336866
60 0.0703748813458732
61 0.0694807787159276
62 0.0616892442239853
63 0.0680662121507534
64 0.0654387905475391
65 0.0670492229434327
66 0.0610851700429599
67 0.0768388189085693
68 0.0584607954875407
69 0.0607771115434937
70 0.0608952010310329
71 0.0667097545164235
72 0.0670667256768238
73 0.0649186199453924
74 0.0556448272726625
75 0.0646885498845683
76 0.0655676398447314
77 0.0604994854525862
78 0.059692714838807
79 0.0578826883491017
80 0.054506333108661
81 0.0535130618163578
82 0.0592184852264757
83 0.0539270788108642
84 0.052963417339726
85 0.0526600471300227
86 0.0555563867506916
87 0.0550974963783857
88 0.0546361086857084
89 0.0547776257216191
90 0.0579173646680528
91 0.0507320531026726
92 0.0602244622247068
93 0.0562640181473424
94 0.0537386058523752
95 0.0604685521598236
96 0.0562264306866779
97 0.0561501914763748
98 0.0556622860084514
99 0.0528321972925178
100 0.0503805200084686
101 0.0565793384189098
102 0.0516293902597347
103 0.0492948830092236
104 0.050714672051576
105 0.052794644247303
106 0.047618736166072
107 0.0510848559255413
108 0.0539415438277319
109 0.0563290794362409
110 0.0474368847329274
111 0.0507707494521769
112 0.0512267124922365
113 0.052710615223285
114 0.0548343738984155
115 0.0471428586432746
116 0.0491788643316464
117 0.0471205604692103
118 0.0487425037525817
119 0.0496737999941632
120 0.0505970140684384
121 0.0547903637221778
122 0.0512322027809605
123 0.0495484679142602
124 0.0430844755583039
125 0.0478405156069579
126 0.048408760234251
127 0.0477439813987446
128 0.0487961453848429
129 0.0459771746022897
130 0.0523033794499169
131 0.0486573119697664
132 0.0449110711921533
133 0.0426085012211916
134 0.0470744814862047
135 0.0462799434404317
136 0.0455526002527012
137 0.0426509845274902
138 0.045889275401774
139 0.0439826729192834
140 0.0451980871993679
141 0.0459181091681925
142 0.046601967125335
143 0.0425803157750052
144 0.0435923447959916
145 0.0450832412117919
146 0.0427837125682605
147 0.0427999098029797
148 0.046192729717466
149 0.0432259020445648
150 0.0434016659676386
151 0.0419932001308807
152 0.0393288694838087
153 0.0425060875439911
154 0.04998078491275
155 0.0457530864055108
156 0.0413780167473744
157 0.0407980609819246
158 0.044805594167677
159 0.0413377965858462
160 0.041044951667402
161 0.0431024854161405
162 0.0413675066966832
};
\addplot [cedline, color4]
table {%
1 0.235703570803833
2 0.216779621921463
3 0.189537013383463
4 0.175697954935254
5 0.166797253797411
6 0.151551247736776
7 0.149893819437524
8 0.141433429501818
9 0.135709156880845
10 0.134093776101003
11 0.126273660213965
12 0.117949285716551
13 0.11561450488322
14 0.112928479883748
15 0.108144524687127
16 0.109194206563193
17 0.104704484982962
18 0.109073927608633
19 0.109429543516752
20 0.106303046098884
21 0.0960449699721397
22 0.0926451064745533
23 0.0928124790794433
24 0.0909211108446008
25 0.0866927457151006
26 0.0796622865451274
27 0.0846801305254083
28 0.0945496130857419
29 0.0963769854524357
30 0.0893211683621535
31 0.0769502060153184
32 0.0799845842944399
33 0.091878449172736
34 0.0730869626238936
35 0.0810866480250802
36 0.0834456155537508
37 0.07242007748535
38 0.0798439450254559
39 0.0782951278902579
40 0.0725419601264699
41 0.0774576261071439
42 0.0705244952460352
43 0.0743427278557747
44 0.0684059380558776
45 0.0710188841033352
46 0.0661357037013921
47 0.0718788032687035
48 0.0717086119386542
49 0.0697693074536379
50 0.0711348353120959
51 0.0704750830880069
52 0.0629981536147096
53 0.0626538951454216
54 0.0618420868841086
55 0.0677703245087643
56 0.0715941718734638
57 0.0607070758015836
58 0.0615056993923789
59 0.0750412051636981
60 0.0587330459969631
61 0.0675099864957324
62 0.0646122067310934
63 0.0648205374556587
64 0.06081489924433
65 0.0604345852246795
66 0.0580387001301891
67 0.0596046464570791
68 0.0593607788884699
69 0.0572399885736353
70 0.054837325880178
71 0.0613484906347571
72 0.0610544382436288
73 0.0581324137292968
74 0.0613389227232618
75 0.0556953661275745
76 0.0532576780760946
77 0.0535743793380398
78 0.0539741378542553
79 0.0564342829092425
80 0.0588522187657525
81 0.0544558742836821
82 0.0549122440639253
83 0.0507379878369267
84 0.0545538427844383
85 0.0540665995925594
86 0.0515997968166362
87 0.0537003781154791
88 0.0534211493163095
89 0.0528038235858573
90 0.0509722512314176
91 0.0501539340618029
92 0.0494697680804554
93 0.0578109687716588
94 0.0534423168876726
95 0.0535595885571088
96 0.049803091914042
97 0.0479879509405582
98 0.0484928660691059
99 0.0519509914714776
100 0.0521886532538566
101 0.0495596935998687
102 0.0554444259671672
103 0.0479503966270116
104 0.0479269758268499
105 0.0483712201162568
106 0.0467799182487965
107 0.0445005671909455
108 0.050222070750915
109 0.0465544633720589
110 0.0527585985502022
111 0.0456037849963866
112 0.0447235176125272
113 0.0485076498489343
114 0.0437549218376612
115 0.0443553423480388
116 0.0476140706302556
117 0.0447701791986405
118 0.0446793272480146
119 0.048437671359899
120 0.0468130739304801
121 0.048663851767579
122 0.0425102817190058
123 0.0422436961447804
124 0.0436596860138005
125 0.0428081850960924
126 0.0435310124674473
127 0.0430488552869226
128 0.0441018699375824
129 0.0433054843141473
130 0.0435584157904651
131 0.0405318399696313
132 0.0436596034831568
133 0.043417099040043
134 0.041361870950213
135 0.0459490218959877
136 0.0413746925452866
137 0.0414976887851232
138 0.0401878745350143
139 0.0402561967780178
140 0.0417094847808039
141 0.0414969444014669
142 0.0449191354520636
143 0.0413497109629982
144 0.0405079136081819
145 0.0406051057166566
146 0.0403152399987905
147 0.0386932242567338
148 0.0387584141862896
149 0.040178350457712
150 0.0386496789974641
151 0.0410167842153071
152 0.0395840342699808
153 0.0387468859966104
154 0.0401504402479194
155 0.0396588609970454
156 0.0370759670774524
157 0.0391928222462288
158 0.0393865410573911
159 0.0418131748577068
160 0.039543262533937
161 0.0389081027121143
162 0.038020175996535
163 0.0383046505744095
164 0.0387638879564392
165 0.0371499017986101
166 0.0375258874104399
};
\addplot [cedline, color5]
table {%
1 0.218152883722891
2 0.206652881518648
3 0.197487725514867
4 0.187443337292308
5 0.191452704871984
6 0.178948999417007
7 0.0467681571708624
8 0.0184287690463866
9 0.0101284893739622
10 0.00793414607240833
11 0.00787441802661193
12 0.00611040151826664
13 0.0235949192080386
14 0.0251562700297389
15 0.00756855798148393
16 0.0104550908704752
17 0.00708009294892453
18 0.00473047130296611
19 0.00436440283991946
20 0.00474848114915732
21 0.00619383886372088
22 0.00579249764709011
23 0.00450765921520302
24 0.00420319322518831
25 0.00376361123951524
26 0.00380009878541415
27 0.00374177007625398
28 0.00242582686764714
29 0.00176238547518209
30 0.00171635711875362
31 0.00234198772938798
32 0.00187605775378369
33 0.00298925873258976
34 0.00118540149041663
35 0.00204910311332868
36 0.00485029994814712
37 0.00324570856208412
38 0.00146368450081935
39 0.002035819708811
40 0.00131947006656374
41 0.00189681088491306
42 0.00234138017374796
43 0.00638904640678678
44 0.00332886501458063
};
\end{axis}

\end{tikzpicture}


==> figures/01-cfls/train/unmarked-reversal.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={\UnmarkedReversal{}},
x grid style={white!69.0196078431373!black},
xmin=-8.95, xmax=209.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.383329892264179,
ytick style={color=black}
]
\addplot [cedline, color0]
table {%
1 0.362199019645059
2 0.358682936465994
3 0.353267701529964
4 0.336087864947245
5 0.328902457138193
6 0.30399760352011
7 0.306878792814829
8 0.31886361179326
9 0.277680335668723
10 0.27726382062132
11 0.272689457410254
12 0.26493344339685
13 0.253417646649543
14 0.239999419143084
15 0.238956400235215
16 0.228397264312848
17 0.226119480265261
18 0.216861899499069
19 0.214678562695799
20 0.200070658402505
21 0.210709641061293
22 0.213170761256648
23 0.185321045772035
24 0.191728546432345
25 0.190082017769591
26 0.18851807234874
27 0.164921684289691
28 0.160477258422347
29 0.158787224310165
30 0.151890508823548
31 0.146987666965778
32 0.167952155798371
33 0.141855496780169
34 0.13360021722317
35 0.142094183655018
36 0.13754584783938
37 0.134923617807133
38 0.118023374577929
39 0.121317787160986
40 0.126780421176951
41 0.107328850731629
42 0.105349793194908
43 0.0979848014146832
44 0.103341282637049
45 0.0949386332240866
46 0.102576068141573
47 0.098940495328022
48 0.0947588468656899
49 0.0957022365905599
50 0.0897393827451772
51 0.0890137098202534
52 0.0853004838856354
53 0.0858781758635098
54 0.0848686442465348
55 0.0948685856713049
56 0.0828667109127018
57 0.078489368959488
58 0.0834326778369279
59 0.0757894122065757
60 0.0901265271955808
61 0.0714165810063849
62 0.0706811663890901
63 0.0821637417190433
64 0.0694530433254371
65 0.0706735014076922
66 0.0892820909407583
67 0.0801508721532032
68 0.072085045959932
69 0.0688127054990232
70 0.087233327424854
71 0.0666094868637472
72 0.0668159809098212
73 0.0656199570911874
74 0.0699019685039656
75 0.0684638393875185
76 0.0611480119615583
77 0.0646905323223043
78 0.0576640065707293
79 0.0752532875522708
80 0.0605451476091752
81 0.0820578004965609
82 0.0578245543366036
83 0.0622500467275092
84 0.0595659329979989
85 0.0500834381970727
86 0.0531883793699814
87 0.0576547946557643
88 0.054904253309618
89 0.0517753134929602
90 0.0521072362279177
91 0.0511556593449313
92 0.0473331941187412
93 0.0452332577096154
94 0.0553340403266598
95 0.0622560335536877
96 0.0502473550760114
97 0.0473343479443481
98 0.0467656582616496
99 0.0443600606569035
100 0.0464978597115265
101 0.0459786080982789
102 0.0461109300443902
103 0.0434193816739322
104 0.0489149152622187
105 0.046336406965996
106 0.0452886020966295
107 0.0400402518905174
108 0.045219999267977
109 0.0433295668279876
110 0.0405808720644941
111 0.0382700958023365
112 0.0422587357127335
113 0.0383741815805992
114 0.0418710901189485
115 0.0414914183355349
116 0.0376575477257446
117 0.0432171131377815
118 0.0425490814859752
119 0.0585718393191347
120 0.036806858867489
121 0.0465771521825401
122 0.0485889989981518
123 0.0459553459699086
124 0.0390503588501468
125 0.0436296388830524
126 0.0409976603778773
127 0.0556270993580253
128 0.0460639492859288
129 0.0379304415717328
130 0.0395915143003855
};
\addplot [cedline, color1]
table {%
1 0.361756805644668
2 0.36427281837383
3 0.357941085214742
4 0.361726060195441
5 0.332768262199649
6 0.32450237966934
7 0.320314436075768
8 0.323805664188486
9 0.303887724446659
10 0.296147943802567
11 0.281075393440161
12 0.267083018237477
13 0.283583001839599
14 0.252016149414509
15 0.253858732022868
16 0.247828709912579
17 0.240681603740358
18 0.227869826951957
19 0.239937383574968
20 0.220576756056868
21 0.225901758226297
22 0.219868367243314
23 0.202846597812122
24 0.216813256584356
25 0.192451301527737
26 0.184764857220232
27 0.177698917722998
28 0.182654312482188
29 0.178441445590447
30 0.172701357687451
31 0.168643164477167
32 0.163463492974279
33 0.148205483299773
34 0.164819186418431
35 0.144165988278444
36 0.133282377526852
37 0.142938898873127
38 0.137386490117327
39 0.128695476575816
40 0.140687089666179
41 0.127419458237068
42 0.123390720471407
43 0.120911757421426
44 0.136639814807077
45 0.132211611839851
46 0.128339993684203
47 0.125767729631491
48 0.109770948130573
49 0.113400455959319
50 0.100441331642205
51 0.113527747348322
52 0.102325430458295
53 0.0980605372272213
54 0.0894815374812066
55 0.0884485629070526
56 0.096668301714136
57 0.0879673820900971
58 0.101861068181044
59 0.084717560138706
60 0.0825083387380153
61 0.0976677650052584
62 0.0834640984675039
63 0.0746103078733248
64 0.0861878646581961
65 0.0978424387644695
66 0.07509616390401
67 0.074791896159802
68 0.0714929769868912
69 0.0728096864562158
70 0.0744488019076089
71 0.069542911277918
72 0.0947662499333344
73 0.069396142187255
74 0.0735779400498699
75 0.0712185941964265
76 0.074291458051057
77 0.0688210326844651
78 0.0752796065917423
79 0.0668686076006388
80 0.0600552407649511
81 0.0660019003710695
82 0.0702426427305429
83 0.0668937729478967
84 0.0676185494243517
85 0.0622964046586735
86 0.0675452144556308
87 0.0857231921766597
88 0.0726584519452459
89 0.0630528829382059
90 0.0578323843244605
91 0.0619396822854306
92 0.0632184328241757
93 0.0624447491645376
94 0.0711325434080278
95 0.0547022679916019
96 0.0546045631588913
97 0.0581410954344724
98 0.0573913877929273
99 0.0488581517901737
100 0.052025168713649
101 0.0543287872551589
102 0.0476183496665266
103 0.0540342371622682
104 0.0509499917743955
105 0.0500926642873672
106 0.0613805713647567
107 0.0549198385996701
108 0.0548109448223157
109 0.0597704923414442
110 0.0447893278767782
111 0.0470774554799758
112 0.0476481518071982
113 0.0540803331102289
114 0.0438835260365489
115 0.0487848089733869
116 0.0424783497843378
117 0.0536469167482589
118 0.0459160804054623
119 0.0469457987496923
120 0.043375628355675
121 0.0494123452255312
122 0.0490996233873684
123 0.0538912040900152
124 0.0382060419083504
125 0.0446638407521972
126 0.0408638923545511
127 0.0453390054421275
128 0.0404447459027537
129 0.0433818764626818
130 0.0389529885363201
131 0.0347902853926454
132 0.0371714712881286
133 0.034681433818273
134 0.0390461917555477
135 0.0320084827081441
136 0.0403322526443003
137 0.0391135901675737
138 0.0407435575235123
139 0.037215401785432
140 0.0353809428487257
141 0.0335995880728854
142 0.039340309871769
143 0.0378026897760486
144 0.0361185801514932
145 0.0372615034475215
};
\addplot [cedline, color2]
table {%
1 0.365213156152486
2 0.357120608197749
3 0.354347604068206
4 0.336418373093648
5 0.340011216514073
6 0.30015571178718
7 0.293156787989081
8 0.274947219286242
9 0.262642764612978
10 0.262965186112735
11 0.255691616053003
12 0.238739842849463
13 0.222249308040495
14 0.207084796785051
15 0.238350977668169
16 0.191462702628116
17 0.2060168617606
18 0.141334905522019
19 0.083966870141525
20 0.0440027872193043
21 0.019350438746785
22 0.0170219789430496
23 0.00654782052240893
24 0.00601796980467778
25 0.00409046028349652
26 0.0137527454375371
27 0.0162871127021076
28 0.00362939852170974
29 0.0119339813143951
30 0.00385321340557915
31 0.00711403481566764
32 0.00639987172651274
33 0.00804169298452212
34 0.0044850514847557
35 0.00287843391861264
36 0.00322965034649109
37 0.00452098861563688
38 0.00663035170829723
39 0.0069535266172428
40 0.00503463611230476
41 0.00342544894922059
42 0.00347852801909987
43 0.00421532134964325
44 0.00519745660940008
45 0.00382584131821134
};
\addplot [cedline, color3]
table {%
1 0.346229415152176
2 0.329268292227453
3 0.314156853116402
4 0.307012576960125
5 0.295518113362063
6 0.293237429796866
7 0.290161595666025
8 0.287289955924985
9 0.291709290690934
10 0.277902764924754
11 0.278562375241259
12 0.271687801178754
13 0.29438660449731
14 0.273791471688517
15 0.262917399500989
16 0.253921779760485
17 0.254752707593107
18 0.249157641750133
19 0.243831470989757
20 0.253130768113938
21 0.241560806693861
22 0.244590113107242
23 0.24491196499119
24 0.234609850875236
25 0.22040244644288
26 0.226996363343547
27 0.228574977158945
28 0.213286786526658
29 0.23501056998624
30 0.218529460582944
31 0.221047800280782
32 0.215587013339371
33 0.216549416702901
34 0.220145247136597
35 0.215606147252212
36 0.195877532969833
37 0.208380438795315
38 0.196199048127155
39 0.198045377349764
40 0.197566168108454
41 0.198826422609032
42 0.203813881755082
43 0.202842487637636
44 0.197223489763416
45 0.192094937814604
46 0.195152107230196
47 0.197860600657877
48 0.183065572352469
49 0.195902604417673
50 0.178207827961044
51 0.188634068587661
52 0.178212541168117
53 0.177756199690705
54 0.183685381209547
55 0.179073204262914
56 0.17974235112432
57 0.169476627449105
58 0.181204777287466
59 0.188759264756528
60 0.176354962359232
61 0.168479984732579
62 0.172628202034141
63 0.169867646723433
64 0.171065354333329
65 0.163907698988167
66 0.167601645829608
67 0.166810392126446
68 0.167298915297283
69 0.160030093599366
70 0.172491150792945
71 0.167682961820429
72 0.162983016277983
73 0.168324139792268
74 0.162386493605102
75 0.157207950320326
76 0.163750115110031
77 0.162662197912168
78 0.157355980927386
79 0.152133215540373
80 0.169495577549044
81 0.168884034919695
82 0.153349579166909
83 0.152726352599468
84 0.155074510228578
85 0.147144843667231
86 0.153128186955552
87 0.144889286949895
88 0.147447417831199
89 0.147149149932124
90 0.15475762357183
91 0.147149288843586
92 0.147400825845714
93 0.145556790804719
94 0.15076603738387
95 0.149227881716665
96 0.140028188533646
97 0.140640851100956
98 0.138602668548755
99 0.144882325638289
100 0.140085757448742
101 0.138761533597013
102 0.134266808002798
103 0.138335945467209
104 0.136797765148203
105 0.136052051859137
106 0.14452034027939
107 0.138191589676746
108 0.13661128366546
109 0.130260940522198
110 0.133142797874032
111 0.131608171799041
112 0.134456540879948
113 0.134223889753191
114 0.129506376089045
115 0.135049637225137
116 0.128572027694019
117 0.127149628192081
118 0.127960561707784
119 0.128947753279116
120 0.125467230421189
121 0.13687874778056
122 0.130779435266346
123 0.128734970283296
124 0.124874387473478
125 0.126491133171714
126 0.130477848381105
127 0.12393335324131
128 0.129039417104928
129 0.123350411570947
130 0.123948210328395
131 0.122822142794298
132 0.126923846565749
133 0.129136942150607
134 0.130405174303793
135 0.121257186046438
136 0.124022279210784
137 0.127715629801913
138 0.133162449158123
139 0.123283975325641
140 0.118860387726844
141 0.118806871287728
142 0.119759806892998
143 0.126382712821016
144 0.118173173286436
145 0.126295060308425
146 0.116934208484013
147 0.123544431352755
148 0.117570122670341
149 0.125893292239808
150 0.114509432839734
151 0.120118020901326
152 0.116902352045016
153 0.12103762704549
154 0.117748028949968
155 0.119607532429442
156 0.117769344105051
157 0.121463299521045
158 0.115379935078922
159 0.119455734617552
160 0.116005660318809
};
\addplot [cedline, color4]
table {%
1 0.351366270077337
2 0.327847758498378
3 0.317798119428304
4 0.311747869532323
5 0.313549167998595
6 0.311912605507893
7 0.306873418766676
8 0.293805354498585
9 0.292546330118119
10 0.287546372616821
11 0.287129339861371
12 0.286393106904322
13 0.279078303105838
14 0.270240686123195
15 0.265721300774663
16 0.265255564661246
17 0.259075751337478
18 0.261190832150727
19 0.252420369332227
20 0.260183773808721
21 0.252378041083162
22 0.244476944598786
23 0.24230188895029
24 0.237060845902688
25 0.238796759640392
26 0.240659931871369
27 0.233097276099863
28 0.229337356115455
29 0.226827469570532
30 0.221429753392342
31 0.228381132992862
32 0.228140651209641
33 0.221710014181359
34 0.219865114385782
35 0.211655404493798
36 0.211812441062772
37 0.205035399712479
38 0.206979851820388
39 0.210132736776596
40 0.226170167237251
41 0.203512342210378
42 0.204780305936555
43 0.206339661389233
44 0.211646599803259
45 0.208400413612269
46 0.199697653934612
47 0.207571108303456
48 0.209585082763153
49 0.203154056241865
50 0.195349626580877
51 0.195060685101185
52 0.188149802043088
53 0.196100828399896
54 0.209261720250404
55 0.195608396352126
56 0.194131302916167
57 0.185526744894232
58 0.18870811737117
59 0.192842910616975
60 0.188632905820296
61 0.184638912023351
62 0.19073629433675
63 0.188786726415535
64 0.186634291832046
65 0.177941159582949
66 0.179125052616034
67 0.173836754686665
68 0.179423012917302
69 0.192498930274502
70 0.175105341253461
71 0.178639152569657
72 0.1743141611476
73 0.176656242778935
74 0.169867295969399
75 0.168169662097313
76 0.172527627621582
77 0.168354381964235
78 0.169391367179141
79 0.177886518762681
80 0.167860016322449
81 0.176082370529548
82 0.165009842482991
83 0.171669105848532
84 0.166417486685157
85 0.173255297674015
86 0.157581896754859
87 0.165558754839093
88 0.162897256134505
89 0.159133248895901
90 0.176353132791836
91 0.166491249022598
92 0.160556734040798
93 0.164371058034198
94 0.164731206281343
95 0.158465386634973
96 0.154683455409229
97 0.162312553329206
98 0.166605054795567
99 0.160329582138525
100 0.16051644219743
101 0.156242409184746
102 0.153276746558985
103 0.157662302600655
104 0.152993438174879
105 0.158391855339171
106 0.150552571684939
107 0.154926181899916
108 0.148510898553213
109 0.148135060874255
110 0.150705291845853
111 0.151629018378752
112 0.155075820069856
113 0.155381169831055
114 0.157674831011581
115 0.146642893812298
116 0.147914175577882
117 0.152992677414591
118 0.149304494826045
119 0.146543220784293
120 0.14506826354344
121 0.146743948778908
122 0.15330537027869
123 0.144529606560179
124 0.147918137764028
125 0.145214505022678
126 0.14373611936509
127 0.155669665558946
128 0.144913982787226
129 0.146269138346977
130 0.14698172173052
131 0.143119008232688
132 0.142113344643247
133 0.145061292490876
134 0.143328664840796
135 0.144336177086051
136 0.147382405095786
137 0.143429357019305
138 0.139665858760987
139 0.138170116122396
140 0.139829150246743
141 0.137809189724821
142 0.141429046789764
143 0.138873060638304
144 0.133909332559441
145 0.14198147328713
146 0.136748965695618
147 0.136018850721238
148 0.138971747662587
149 0.141207444870079
150 0.138065593555798
151 0.146018660029224
152 0.130334406707039
153 0.13220951212591
154 0.146233140736741
155 0.131788997147784
156 0.13318927414232
157 0.140342398666456
158 0.135495072965807
159 0.132779333506707
160 0.144297458795411
161 0.126523195260293
162 0.126664789397481
163 0.135592827170362
164 0.127182282448429
165 0.1299949854033
166 0.139940495544357
167 0.131909222872787
168 0.138125261906487
169 0.127464909390732
170 0.126094171879254
171 0.132617921784048
172 0.133663988456057
173 0.127095910252699
174 0.135719421906196
175 0.124655814402874
176 0.124168403926609
177 0.132022654105542
178 0.125169085633312
179 0.126057937966752
180 0.12515934333038
181 0.134644863032449
182 0.12757004921722
183 0.132237262436806
184 0.121742338247509
185 0.126789182546163
186 0.122090492242961
187 0.125658069952688
188 0.128407084278746
189 0.12103745478231
190 0.129427256861391
191 0.121973075159011
192 0.121422115066274
193 0.122465763511364
194 0.123720422998035
195 0.119637779520216
196 0.127317113198077
197 0.11490521478379
198 0.119150563460371
199 0.118123571330869
200 0.121480143945186
};
\addplot [cedline, color5]
table {%
1 0.348738821532208
2 0.350707603570268
3 0.326424539621788
4 0.308223796476918
5 0.299513850594284
6 0.293528812556043
7 0.291031071031627
8 0.285222982428093
9 0.283727835153845
10 0.285246643944639
11 0.279628456642412
12 0.271087304488127
13 0.270480939471366
14 0.261445077411251
15 0.268182761565948
16 0.258132602127152
17 0.248708118688816
18 0.244375872213376
19 0.246614529184501
20 0.227335780284375
21 0.217484092976472
22 0.222223360217323
23 0.208673780442552
24 0.20891910583589
25 0.200264999901643
26 0.196043496416641
27 0.193636785315763
28 0.187273939731914
29 0.184227090767936
30 0.175445937743893
31 0.17044927485411
32 0.171238548474631
33 0.170137080369725
34 0.163955241706784
35 0.162586079750112
36 0.159275452793371
37 0.176490171735533
38 0.163254856486854
39 0.160369421323472
40 0.149829719704114
41 0.149795957774896
42 0.145903132754792
43 0.134803905458572
44 0.14121763453816
45 0.132928020602597
46 0.13534034449697
47 0.133921458192046
48 0.125938501835754
49 0.122889529223576
50 0.126179164774741
51 0.132114556882208
52 0.117373048397678
53 0.119806105878788
54 0.124901345495656
55 0.116525281201811
56 0.113655318901622
57 0.1150944583008
58 0.11935566246796
59 0.124209903767277
60 0.113730007882731
61 0.103895248853416
62 0.104364558833121
63 0.116323732957224
64 0.114094729755385
65 0.105421626175938
66 0.0998398702979663
67 0.100946665801824
68 0.105590458710259
69 0.0979278300460157
70 0.094476154047948
71 0.0975630183640149
72 0.094135052894491
73 0.0931528838195679
74 0.102693410742332
75 0.0882952635484536
76 0.101739660625912
77 0.0947984960078392
78 0.0786571048027671
79 0.0839976449337386
80 0.0872743570527754
81 0.0733295857790849
82 0.0723006345259678
83 0.0883811785075456
84 0.0649361490086454
85 0.0680675433643459
86 0.0606126137457228
87 0.0617143509338445
88 0.061388677672451
89 0.0625364846912775
90 0.0550485293790713
91 0.0581324178153702
92 0.0534620489508109
93 0.0506568547016612
94 0.0475395558153214
95 0.0477993816596062
96 0.0458667299972014
97 0.0501741534991743
98 0.0455878204807167
99 0.0540139642780542
100 0.0508359572953653
101 0.0475951120548708
102 0.042117695915004
103 0.0530050372157582
104 0.0405776575239123
105 0.0476296600157732
106 0.0534019982197823
107 0.0327884293789448
108 0.0366935056381184
109 0.0377052616628936
110 0.0334796289468088
111 0.0436674170535357
112 0.0475397866648079
113 0.0334151663343603
114 0.032720876351452
115 0.0348107189337265
116 0.0556768151542393
117 0.035742082874229
118 0.0382965400560537
119 0.0325806794953107
120 0.0367351218775122
121 0.0299534526765641
122 0.03383979389626
123 0.0354488077120425
124 0.0357722154118477
125 0.0437118338831647
126 0.0324143703850354
127 0.0347031620492808
128 0.0353068116972729
129 0.0287539650360559
130 0.0280437189320145
131 0.0296917678422211
132 0.0366374960025795
133 0.02802692733271
134 0.0443329220583813
135 0.0352262630315016
136 0.0346059612036114
137 0.027650297717503
138 0.0287408706391364
139 0.0276756514859751
140 0.0292372400271627
141 0.0391081917068262
142 0.0248901964369265
143 0.0363363904527733
144 0.0311353113328307
145 0.0465182178802053
146 0.0278496567553125
147 0.0290674736741638
148 0.0285671772375081
149 0.0389011298088592
150 0.0234685027817229
151 0.0334021328314286
152 0.0242898327599256
153 0.0361291429291082
154 0.027102248038237
155 0.0308914619091493
156 0.0354424210506315
157 0.0204722317256502
158 0.0206972933725028
159 0.0291743843774144
160 0.0216770294435844
161 0.0254510237691022
162 0.0196711800652887
163 0.0239520534398838
164 0.0256333606296408
165 0.0268931562522296
166 0.0272042645609969
167 0.0273262937510959
168 0.0296270605833994
169 0.0267678530349743
170 0.0256637206570961
171 0.0262446308546379
172 0.0298923650680647
};
\end{axis}

\end{tikzpicture}

